A stable and adaptive semi-Lagrangian potential model for unsteady and nonlinear ship-wave interactions

We present an innovative numerical discretization of the equations of inviscid potential flow for the simulation of three dimensional unsteady and nonlinear water waves generated by a ship hull advancing in water. The equations of motion are written in a semi-Lagrangian framework, and the resulting integro-differential equations are discretized in space via an adaptive iso-parametric collocation Boundary Element Method, and in time via adaptive implicit Backward Differentiation Formulas (BDF) with variable step and variable order. When the velocity of the advancing ship hull is non-negligible, the semi-Lagrangian formulation (also known as Arbitrary Lagrangian Eulerian formulation, or ALE) of the free surface equations contains dominant transport terms which are stabilized with a Streamwise Upwind Petrov-Galerkin (SUPG) method. The SUPG stabilization allows automatic and robust adaptation of the spatial discretization with unstructured quadrilateral grids. Preliminary results are presented where we compare our numerical model with experimental results on the case of a Wigley hull advancing in calm water with fixed sink and trim.

==> paper.tex <==
\input{Preamble.tex}

\date{}

\begin{document}
\begin{frontmatter}

  \title{A stable and adaptive semi-Lagrangian potential model for
    unsteady and nonlinear ship-wave interactions}

  \author[Sissa]{Andrea Mola}
  \ead{andrea.mola@sissa.it}
  \author[Sissa,cor]{Luca Heltai} 
  \ead{luca.heltai@sissa.it}
  \author[Sissa]{Antonio DeSimone} 
  \ead{desimone@sissa.it}
  % 
  \cortext[cor]{Corresponding author, Tel.: +39 040-3787449; Fax: +39 040-3787528}

  \address[Sissa]{SISSA, International School for Advanced Studies, \\ 
    Via Bonomea 265, 34136 Trieste - Italy} 


  \begin{abstract}


    We present an innovative numerical discretization of the equations of
    inviscid potential flow for the simulation of three dimensional
    unsteady and nonlinear water waves generated by a ship hull advancing
    in water.  

    The equations of motion are written in a semi-Lagrangian framework,
    and the resulting integro-differential equations are discretized in
    space via an adaptive iso-parametric collocation Boundary Element
    Method, and in time via adaptive implicit Backward Differentiation
    Formulas (BDF) with variable step and variable order.

    When the velocity of the advancing ship hull is non-negligible, the
    semi-Lagrangian formulation (also known as Arbitrary Lagrangian
    Eulerian formulation, or ALE) of the free surface equations contains
    dominant transport terms which are stabilized with a Streamwise Upwind
    Petrov-Galerkin (SUPG) method.

    The SUPG stabilization allows automatic and robust adaptation of the
    spatial discretization with unstructured quadrilateral
    grids. Preliminary results are presented where we compare our
    numerical model with experimental results on the case of a Wigley hull
    advancing in calm water with fixed sink and trim.
  \end{abstract}
   \begin{keyword}
     unsteady ship-wave interaction; nonlinear free surface problems; semi-Lagrangian
     formulation; arbitrary Lagrangian Eulerian formulation; boundary element method 
   \end{keyword}
\end{frontmatter}

%\tableofcontents

%\listoffixmes
\clearpage

\section{Introduction}

Over the last decades, the need for accurate prediction of the
hydrodynamic performances of ships has led to the development of
increasingly efficient and accurate models for the simulation of the
three dimensional, nonlinear and unsteady water waves generated by a
moving hull. In particular, models based on potential flow theory have
historically been among the most successful in the simulation of the
dynamics of nonbreaking waves. In this framework, the assumptions of
irrotational flow and inviscid fluid reduce the Navier Stokes
incompressibility constraint and momentum balance equations to the
Laplace's and Bernoulli's equations, defined on a moving domain.

This boundary value problem is tackled with a Mixed
Eulerian--Lagrangian approach, in which the Eulerian field equations
are solved to obtain the fluid velocities, which are then used to
displace in a Lagrangian way the free surface, and update the
corresponding potential field values \cite{tanizawa2000}. In this
framework, the Eulerian problem is expressed in boundary integral
form, and it is typically discretized using the Boundary Element
Method (BEM).
% \LH{? Remove
%   from here} Allowing for the discretization of the boundary of the
% domain only, such method presents, for the problem at hand, several
% advantages with respect to other discretization methodologies. First,
% discretizing only the boundaries of the domain leads to a significant
% reduction of the degrees of freedom of the problem, with consequent
% reduction of the computational cost of the simulations. For the same
% reason, the simulation data storage requirements are very small,
% making flow visualizations and data analysis particularly simple.  But
% more importantly, the surface meshes needed for BEM are of much
% simpler generation and deformation with respect to three dimensional
% grids, making this method particularly suitable for problems with
% moving boundaries, such as the one considered here. \LH{to here?}
%
The velocity field and Bernoulli's equation provide a kinematic
boundary condition for the Lagrangian evolution of the free surface,
and a dynamic boundary condition for the evolution of the potential
field.

Numerical treatments of the Lagrangian step usually rely on accurate
reconstructions of position vector and potential field gradients,
which may lead to instability in the time advancing scheme for the
free surface discretization, as well as for the corresponding
potential field values. A smoothing technique is typically adopted to
reduce the sensitivity of the discretization on the reconstruction of
the full velocity field, at the cost of introducing an artificial
viscosity in the system.

An alternative cure was presented by Grilli et al. \cite{grilli2001}
who developed a high order iso-parametric BEM discretization of a
Numerical Wave Tank to simulate overturning waves up to the breaking
point on arbitrarily shaped bottoms. The use of a high order
discretization bypasses the problem of reconstructing the gradients,
and is very reliable when the numerical evolution of the free surface
is done in a purely Lagrangian way.

Ship hydrodynamics simulations, however, are typically carried out in
a frame of reference attached to the boat, requiring the presence of a
water current in the simulations, which, in a fully Lagrangian
approach, leads to downstream transportation of the free surface
nodes, or to their clustering around stagnation points, ultimately
resulting in blowup of the simulations (see, for example,
\cite{scorpioPhD}).

Beck~\cite{beck1994} proposed alternative \emph{semi-Lagrangian} free
surface boundary conditions, under the assumption that the surface
elevation function is single-valued. Employing such conditions, it is
possible to prescribe the horizontal velocity of the free surface
nodes of the computational grid, and compute the vertical velocity
needed to keep the nodes on the free surface. However, in presence of
significant difference between the water current speed and the
horizontal nodes speed, the semi-Lagrangian scheme has some dominant
transport terms, and stability issues may arise \cite{scorpioPhD},
\cite{RyuKimLynett2003}. The semi-Lagrangian free surface boundary
conditions proposed by Beck have been in most cases employed imposing
nodes longitudinal speeds equal to the water current ones, and lateral
velocities chosen so that the nodes would follow prescribed horizontal
paths \cite{scorpioPhD}. %\cite{otherBeckStuff}

More recently, Sung and Grilli \cite{SungGrilli2008} applied an
alternative method, combining semi-Lagrangian and Lagrangian free
surface boundary conditions to the problem of a pressure perturbation
moving on the water surface, which was then tested on a Wigley
hull. The semi-Lagrangian free surface boundary conditions were used
also in the work of Kjellberg, Contento and Jansson
\cite{KjelContJans-2011}, where free surface instabilities are
avoided by choosing an earth fixed reference frame, in which no
current speed is needed. The drawback of this choice is that in such
frame the ship moves with a specified horizontal speed, and the
computational grid needs to be constantly regenerated to cover the
region surrounding the hull with an adequate number of cells.

The purpose of this work is to present new results obtained with a
semi-Lagrangian potential model for the simulation of three
dimensional unsteady nonlinear water waves generated by a ship hull
advancing in calm water. The resulting integro-differential boundary value
problem is discretized to a system of nonlinear differential-algebraic
equations, in which the unknowns are the positions of the nodes of the
computational grid, along with the corresponding potential and
potential normal derivative values. Among these, the vertical
positions and the potential values associated with the free surface
nodes are differential components, while the other unknowns are purely
algebraic.

Time advancing of the nonlinear differential-algebraic system is
performed using implicit Backward Differentiation Formulas (BDF) with
variable step size and variable order. At each time step, such method
results in a nonlinear algebraic system, solved with Newton's
method. Both the BDF and Newton's method are implemented in the
framework of the open source library SUNDIALS \cite{sundials2005} for
the resolution of nonlinear differential-algebraic equations. The
collocated and iso-parametric BEM discretization of the Laplace's
equation has been implemented employing the open source C++ library
deal.II \cite{BangerthHartmannKanschat2007}.

The computational grid, composed by quadrilateral cells of arbitrary
order, is adapted in a geometrically consistent way
(see~\cite{BonitoNochettoPauletti-2010-a}) via an a posteriori error
estimator based on the jump of the solution gradient along the cell
internal boundaries. Even when low order boundary elements are used,
accurate estimations of the position vector and potential gradients on
the free surface are recovered by means of a Streamwise Upwind
Petrov--Galerkin (SUPG) projection, which is used to stabilize the
transport dominated terms. The SUPG projection is strongly consistent,
and does not introduce numerical dissipation in the equations,
allowing the use of robust unstructured grids, which can be generated
and managed on arbitrary hull geometries in a relatively simple way.

The test case considered in this paper is that of a Wigley hull
advancing at constant speed in calm water. The simulations have been
performed using bilinear elements. The arbitrary horizontal velocity
specified in the semi-Lagrangian free surface boundary condition is
chosen so as to impose null longitudinal nodes velocity with respect
to the hull. The simulations results obtained imposing six different
Froude numbers are finally compared with experimental results reported
in \cite{mccarthy1985}, to assess the accuracy of the model.



\section{Three dimensional potential model}

The equations of motion that better describe the velocity and pressure
fields $\vb$ and $p$ of a fluid region around a ship hull are the
incompressible Navier--Stokes equations, written in the moving domain
$\Omega(t) \subset\mathbb{R}^3$, which is a (simply connected) region
of water surrounding the ship hull itself:


%.  When viscosity is neglected,
%they reduce to the incompressible Euler equations in the moving domain
%$\Omega(t) \subset\mathbb{R}^3$, which is a (simply connected) region
%of water surrounding the ship hull itself:

\begin{subequations}
  \label{eq:incompressible-euler}
  \begin{alignat}{3}
    \label{eq:conservation-momentum}
    & \rho \left( \frac{\partial \vb}{\partial t} + \vb \cdot \nablab
    \vb \right)= \nablab\cdot\sigmab + \bb \qquad & \text{ in } \Omega(t)\\
    \label{eq:incompressibility}
    & \nablab \cdot \vb = 0 & \text{ in } \Omega(t)\\
    \label{eq:freesurface-condition}
    & \sigmab\cdot\nb = p_a \nb & \text{ on } \Gamma^w(t)\\
    \label{eq:non-penetration-condition}
    & \vb = \vb_g & \text{ on } \Gamma(t)\setminus
    \Gamma^w(t)
  \end{alignat}
\end{subequations}
where $\rho$ is the (constant) fluid density, $\bb$ are external body
forces (typically gravity and possibly other inertial forces due to a
non inertial movement of the reference frame), $\sigmab = -p\Ib +
\mu(\nablab\vb+\nablab\vb^T)$ is the stress tensor for an
incompressible Newtonian fluid, $\Gamma(t) := \partial\Omega(t)$ is
the boundary of the region of interest, and $\nb$ is the outer normal
to the boundary $\Gamma(t)$. On the free surface $\Gamma^w(t)$, the
air is assumed to exert a constant atmospheric pressure $p_a$ on the
underlying water, and we neglect shear stresses due to the wind. On
the other boundaries of the domain, the prescribed velocity $\vb_g$ is
either equal to the ship hull velocity, or to a given velocity field
(for inflow and outflow boundary conditions far away from the ship
hull itself).

Equation~(\ref{eq:conservation-momentum}) is usually referred to as
the momentum balance equation, while (\ref{eq:incompressibility}) is
referred to as the incompressibility constraint, or continuity
equation.

In the flow field past a slender ship hull, vorticity is confined to
the boundary layer region and to a thin wake following the boat: in
these conditions, the assumption of irrotational and non viscous flow
is fairly accurate, and viscous effects can be recovered, if necessary,
by other means such as empirical algebraic formulas, or ---better--- by
the interface with a suitable boundary layer model.

For an irrotational and invishid flow, the velocity field $\vb$
admits a representation through a scalar potential function
$\Phi(\xb,t)$, namely
\begin{equation}
\label{eq:potential-definition}
\vb = \nablab\Phi \qquad\qquad    \text{in} \ \ \Omega(t).
\end{equation}
%
In this case, the equations of motion simplify to the unsteady
Bernoulli equation and to the Laplace equation for the flow potential:

\begin{subequations}
  \label{eq:incompressible-euler-potential}
  \begin{alignat}{3}
    \label{eq:bernoulli}
    & \frac{\Pa\Phi}{\Pa t}+\frac{1}{2}\left|\nablab\Phi\right|^2
      +\frac{p-p_a}{\rho}+\bbeta
      \cdot \xb = C(t) \qquad & \text{ in } \Omega(t)\\
    \label{eq:incompressibility-potential}
    & \Delta \Phi = 0 & \text{ in } \Omega(t)
  \end{alignat}
\end{subequations}
% 
where $C(t)$ is an arbitrary function of time, and we have assumed
that all body forces could be expressed as $\bb = -\nablab (\bbeta
\cdot \xb)$, i.e., they are all of potential type. This is true for
gravitational body forces and for inertial body forces due to uniform
accelerations along fixed directions of the frame of reference.

In this framework, the unknowns of the problem $\Phi$ and $p$ are
uncoupled, and it's possible to recover the pressure by postprocessing
the solution of the Poisson
problem~(\ref{eq:incompressibility-potential}) via Bernoulli's
Equation~(\ref{eq:bernoulli}). 

Since arbitrary uniform variations of the potential field produce the
same velocity field (i.e., $\nablab(\Phi(\xb, t)+C(t)) =
\nablab\Phi(\xb, t)$), we can set $C(t)=0$, and we can combine
Bernoulli equation~(\ref{eq:bernoulli}) and the dynamic boundary
condition on the free surface~(\ref{eq:freesurface-condition}) to
obtain an evolution equation for the potential field $\Phi(\xb,t)$ on
the free surface $\Gamma^w(t)$.

The shape of the water domain $\Omega(t)$ is time dependent and it is
part of the unknowns of the problems. The free surface $\Gamma^w(t)$
should move following the fluid velocity $\vb$.  In ship
hydrodynamics, however, it is desirable to maintain the frame of
reference attached to the boat, and study the problem in a domain
which is neither fixed nor a material subdomain, since its evolution
is not governed solely by the fluid motion, but also by the motion of
the reference frame and by the motion of the stream of
water. Nonetheless, it has to comply to the free surface boundary
$\Gamma^w(t)$ which is the result of the dynamic boundary
condition~(\ref{eq:freesurface-condition}).

A possible solution is to introduce an intermediate frame of
reference, called Arbitrary Lagrangian Eulerian (ALE) (see, for
example, \cite{formaggia2009cardiovascular}). This approach is also
known, in the context of potential free surface flows, as the
\emph{semi-Lagrangian} approach~\cite{BeckCaoLee-1993-a,scorpioPhD}.

\subsection{Arbitrary Lagrangian Eulerian Formulation}
\label{sec:ale}

\begin{figure}[htb!]
  \centering
  \xfig[1]{ALE}
  \caption{Schematic representation of a Lagrangian motion and of an arbitrary
    Lagrangian Eulerian motion.}
  \label{fig:lag-ale-motions}
\end{figure}

% As simple a statement as this may seem, there are some issues that
% arise if one tries to express these conditions in a purely Eulerian
% framework. As the water elevation changes close to the hull, there is
% also an exchange of roles between free surface locations and ship hull
% locations, i.e., points on $\Gamma^w(t)$ may end up being on
% $\Gamma^h(t)$, and viceversa, making it necessary to change the
% computational grid at each time, either by reconstructing it at each
% time or by some sort of deformation of the original computational
% grid.

% An alternative approach to the purely Eulerian description is the
% purely Lagrangian one, in which the boundary value problem is defined
% on a fixed reference domain made of fluid particles, which are then
% followed during their evolution in time. While this approach
% eliminates at once the issue of exchanging free surface and hull
% locations, it is still not applicable \emph{as is} to ship
% hydrodynamic simulations, since fluid particles would be constantly
% streaming away from the location of the ship hull, making it
% unpractical for long time simulations \AM{Maybe cite people doing this
% anyway?}.

A \emph{motion} is a time parametrized family of invertible maps which
associates to each point $\xlag$ in a reference domain $\Olag$ its
position in space at time $t$:
\begin{equation}
  \label{eq:lagrangian-motion}
  \plag: \Olag\times\Re \mapsto \Re^3, \qquad (\xlag,t) \mapsto
  \xb=\plag(\xlag, t).
\end{equation}
The domain $\Omega(t)$ at the current time can be seen as the image
under the motion $\plag$ of a reference domain $\Olag$, i.e., 
$\plag(\Olag,t)=\Omega(t)$. We will indicate with the $\hat \cdot$
symbol a \emph{material motion}, or a motion in which the points
$\xlag$ label material particles.

If one does not want to follow material particles with the domain
$\Omega(t)$, it is possible to introduce another intermediate motion,
called the \emph{ALE motion}, with which we represent deformations of
the domain $\Omega(t)$:
\begin{equation}
  \label{eq:ale-motion}
  \pale: \Oale\times\Re \mapsto \Re^3, \qquad (\xale,t) \mapsto
  \xb=\pale(\xale, t).
\end{equation}
These motions can be rather arbitrary, as long as the \emph{shape} of
the domain $\Omega(t)$ is preserved by the motion itself, i.e.,
$\pale(\Oale,t) = \Omega(t)$. The points labelled with $\xale$ do not,
in general, represent material particles. See
Figure~\ref{fig:lag-ale-motions} for a schematic representation of a
Lagrangian motion and of an ALE motion. 

Given a Lagrangian field $\qlag:\Olag\times\Re\mapsto\Re$, its
Eulerian representation is 
\begin{equation*}
  q(\xb,t) := \qlag(\plag^{-1}(\xb,t), t), \qquad \forall \xb \in \Omega(t),
\end{equation*}
while, given an Eulerian field $q:\Omega(t)\times \Re\mapsto \Re$, its
Lagrangian representation would be
\begin{equation*}
  \qlag(\xlag,t) := q(\plag(\xlag,t), t), \qquad \forall \xlag \in \Olag.
\end{equation*}
%
A similar structure is valid for ALE fields:
\begin{alignat*}{2}
  q(\xb,t) &:= \qale(\pale^{-1}(\xb,t), t), \qquad &\forall \xb \in
  \Omega(t),\\
  \qale(\xale,t) &:= q(\pale(\xale,t), t), &\forall \xale \in \Oale.
\end{alignat*}

The fluid particle velocity $\vb$ which appears in
Problem~(\ref{eq:incompressible-euler}) is the Eulerian
representation of the particles velocity
\begin{equation*}
  \vb(\plag(\xlag,t), t) = \hat\vb(\xlag,t) := \frac{\Pa \plag(\xlag,t)}{\Pa t}.
\end{equation*}
%
In a similar way, we define the Eulerian representation of the
\emph{domain velocity}, or \emph{ALE velocity} the field $\wb$ such
that
\begin{equation*}
  \wb(\pale(\xale,t), t) = \hat\wb(\xale,t) := \frac{\Pa \pale(\xale,t)}{\Pa t}.
\end{equation*}

Time variations of physical quantities associated with material
particles are computed at fixed $\xlag$, generating the usual material
derivative
\begin{equation*}
  \frac{D q(\xb,t)}{Dt} := \left.\frac{\partial q(\plag(\xlag,t),t)}{\partial t}
  \right|_{\xlag=\plag^{-1}(\xb,t)} = \frac{\Pa q(\xb,t)}{\Pa t}+\vb \cdot
  \nablab q(\xb,t).
\end{equation*}
%
In a similar fashion, if we compute quantities at fixed ALE point
$\xale$, we obtain the ALE time derivative, wich we will denote as
\begin{equation*}
  \frac{\delta q(\xb,t)}{\delta t} := \left.\frac{\partial q(\pale(\xale,t),t)}{\partial t}
  \right|_{\xale=\pale^{-1}(\xb,t)} = \frac{\Pa q(\xb,t)}{\Pa t}+\wb \cdot
  \nablab q(\xb,t).
\end{equation*}

The ALE deformation allows one to define the equations of motions in
Problem~(\ref{eq:incompressible-euler}) in terms of the fixed ALE
reference domain $\Oale$, while still solving the same physical
problem. On the free surface part of the boundary, the ALE motion
needs to follow the evolution of the fluid particles in order to
maintain the correct shape of the domain $\Omega(t)$, in particular
the minimum requirement for the ALE motion on the free surface is
given by the \emph{free surface kinematic boundary condition}
\begin{equation}
  \label{eq:freesurface-kinematic-condition}
  \wb\cdot\nb = \vb\cdot\nb \qquad \text{ on }\Gamma^w(t),
\end{equation}
which complements the dynamic boundary
condition~(\ref{eq:freesurface-condition}), and provides an evolution
equation for the normal part of the ALE motion on the boundary
$\Gamma^w(t)$. In terms of the ALE motion, the above condition reads
\begin{equation}
  \label{eq:freesurface-kinematic-condition-ale}
  \frac{\Pa\pale}{\Pa t}(\xale, t) \cdot \nb = \vb(\pale(\xale, t),
  t)\cdot\nb \qquad \text{ on }\Gamma^w(t).
\end{equation}

Equations~(\ref{eq:freesurface-condition})
and~(\ref{eq:freesurface-kinematic-condition}) are usually referred to
as the free surface dynamic and kinematic boundary conditions, since
they represent the physical condition applied to the free surface
(equilibrium of the pressure on the water surface) and its evolution
equation (the shape of the free surface follows the velocity field of
the flow).


\subsection{Perturbation potential and boundary conditions}

\begin{figure}[htb!]        
\centerline{\xfig[0.8]{dominio_barca}}
\caption{The domain $\Omega(t)$ and the different regions
         in which its boundary $\Pa\Omega(t)$ is split. The grey area
         behind the hull $\Gamma^{h}(t)$, is the absorbing beach portion
         of the free surface region $\Gamma^{w}(t)$.  
         \label{fig:wholeDomain}}	
\end{figure} 

In the context of moving ship hulls, it is desirable to maintain the
frame of reference of the domain $\Omega(t)$ around the region where
the boat is moving, i.e., we want to solve Problem
(\ref{eq:incompressible-euler-potential}) in a local frame of reference
translating with uniform horizontal speed
$\Vb_{\sys}(t)$. Similarly, one could be interested in studying
the behavior of the ship hull in the presence of an horizontal water
stream velocity $\Vb_{\stream}(t)$, expressed in a global (earth
fixed) reference frame.

Uniform accelerations of the reference frame can be taken into account
by incorporating them in the body force term
\begin{equation}
  \label{eq:forcing-term}
  \bbeta\cdot\xb = \ab_{\sys}\cdot\xb + gz,
\end{equation}
%
and it is convenient to split the potential $\Phi$ into the sum between
a mean flow potential (due to the stream velocity and to the frame of
reference velocity) and the so called \emph{perturbation potential}
$\phi$ due to the presence of the ship hull, namely

\begin{subequations}
  \begin{alignat}{1}
    \Phi(\xb,t) &= \big(\Vb_{\stream}(t)-\Vb_{\sys}(t)\big)\cdot\xb +
    \phi(\xb,t)\\
    \vb(\xb,t) = \nablab\Phi(\xb,t) &= \Vb_{\stream}(t)-\Vb_{\sys}(t) +
    \nablab\phi(\xb,t)\\
    \frac{\Pa\Phi}{\Pa t}(\xb,t) &=
    \big(\ab_{\stream}(t)-\ab_{\sys}(t)\big)\cdot\xb +
    \frac{\Pa\phi}{\Pa t}(\xb,t).
  \end{alignat}
  \label{eq:potSplit}
\end{subequations}
% 
The perturbation potential still satisfies Poisson equation

\begin{equation*}
\Delta\phi = 0 \qquad\qquad \text{in} \ \ \Omega(t),
\end{equation*}
%
and in practice it is convenient to solve for $\phi$, and obtain the
total potential $\Phi$ from equation (\ref{eq:potSplit}).

In Figure~\ref{fig:wholeDomain} we present a sketch of the domain
$\Omega(t)$, with the explicit splitting of the various parts of the
boundary $\Gamma(t)$. On the boat hull surface, the non penetration
condition takes the form

\begin{equation*}
\phin := \nablab\phi\cdot \nb= \nb\cdot(\Vb_{\boat}-\Vb_{\stream})
\qquad\qquad \text{on} \ \ \Gamma^{h}(t),
\end{equation*}
%
when expressed in terms of the perturbation potential and
$\Vb_{\boat}$ is the (given) boat velocity. % (in this work, we assume
% that the boat is only translating, but the extension to cases in which the hull
% presents nonzero angular velocities is straightforward)


On the ---horizontal--- bottom of the water basin $\Gamma^{b}$, the
non penetration condition is also applied, namely

\begin{equation*}
\phin = 0 \qquad\qquad \text{on} \ \ \Gamma^{b}(t).
\end{equation*}
%
A possible condition for the ---vertical--- far field boundary is the
homogeneous Neumann condition


\begin{equation*}
\phin = 0 \qquad\qquad \text{on} \ \ \Gamma^{ff}(t).
\end{equation*}
%
The most remarkable limit of such condition is the fact that it
reflects wave energy back in the computational domain, thus limiting
the simulation time. Different boundary conditions can be used to let
the wave energy flow outside the domain. We employ an \emph{absorbing
  beach} technique (see, for example, \cite{CaoBeckSchultz-1993}), in
which we add an artificial damping region away from the boat, used to
absorb the wave energy. A damping term can be seen as an additional
pressure $P$ acting on the free surface. In such case, Bernoulli
equation on the free surface becomes

\begin{equation}
\frac{\Pa\Phi}{\Pa t}+gz- \ab_{\stream}\cdot\xb +\frac{1}{2}|\nablab\Phi|^2 + \frac{P}{\rho} = 0
\qquad\qquad \text{ on } \ \ \Gamma^w(t),
\label{eq:bernoulliDamp}
\end{equation}
%
and one can show that the resulting rate of energy absorption is

\begin{equation}
\frac{dE_f}{dt} = \int_{\Gamma^w}P\phin\d\Gamma.
\label{eq:dampRate}
\end{equation}
%
A natural way to construct the damping pressure $P$ is then to use a
term which is proportional to the potential normal derivative
$\phin$, which grants a positive energy absorption at
all times.

The dynamical free surface boundary condition modified to account for the damping
term reads 
%
\begin{equation}
\frac{\Pa\Phi}{\Pa t}+gz- \ab_{\stream}\cdot\xb +\frac{1}{2}|\nablab\Phi|^2 -
\mu\phin = 0
\qquad\qquad \text{ on } \ \ \Gamma^w(t),
\label{eq:fsDynamicBeckDamped}
\end{equation}
%
where
%
\begin{equation}
\mu = \left(\frac{\max\left(0,x-x_d\right)}{L_d}\right)^2,
\end{equation}
%
and $x_d$ is the $x$ coordinate value in which the artificial
damping starts to act, while $L_d$ is the length of the absorbing
beach, as in Figure~\ref{fig:wholeDomain}.


Applying the potential splitting~(\ref{eq:potSplit}) to
Problem~(\ref{eq:incompressible-euler-potential}), and summarizing all
boundary conditions, we obtain the perturbation potential formulation

\begin{subequations}
  \label{eq:incompressible-euler-perturbation-potential}
  \begin{alignat}{2}
    % \label{eq:bernoulli-phi}
    % & \frac{\Pa\phi}{\Pa t} +\vb\cdot\nablab\phi = -gz +
    % \ab_{\stream}\cdot\xb +
    % \frac{1}{2}\left|\nablab\phi\right|^2 &-\frac{p-p_a}{\rho} \qquad \text{in } \Omega(t)\\
    \label{eq:incompressibility-potential-perturbation-phi}
    & \Delta \phi = 0 & \text{ in } \Omega(t)\\
    \label{eq:fsDynamicLag}
    & \frac{\Pa\phi}{\Pa t} +\vb\cdot\nablab\phi= -gz +
    \ab_{\stream}\cdot\xb+ \frac{1}{2}|\nablab\phi|^2 & -
    \mu\phin \qquad \text{ on } \Gamma^w(t) \\
    &\phi(\xb, 0) = \phi_0(\xb) &\text{ on } \Gamma^w(0)\label{eq:initial-condition-phi} \\
    \label{eq:non-penetration-condition-hull}
    &\phin =
    \nb\cdot(\Vb_{\boat}-\Vb_{\stream}) & \text{ on }
    \Gamma^{h}(t)\\
    &\phin = 0 & \text{ on }
    \Gamma^b(t)\cup\Gamma^{ff}(t)\\
    \label{eq:fsKinematicLag}
    &\wb\cdot \nb = \vb\cdot \nb&
    \text{ on }\tilde\Gamma^w(t),
  \end{alignat}
\end{subequations}
where $\vb = \Vb_{\stream} - \Vb_{\sys}+ \nablab\phi$.
Equation~(\ref{eq:fsKinematicLag}) is the kinematic boundary condition
for the evolution of the free surface parametrization, while
Equation~(\ref{eq:fsDynamicLag}) is a dynamic Dirichlet boundary
condition for the Poisson
problem~(\ref{eq:incompressibility-potential-perturbation-phi}) at
each time $t$, whose initial condition is given by
Equation~(\ref{eq:initial-condition-phi}).

% In view of the discretization of
% Problem~(\ref{eq:incompressible-euler-perturbation-potential}), it is
% important to make some considerations. While the Eulerian formulation
% (of which
% Problems~(\ref{eq:incompressible-euler}),~(\ref{eq:incompressible-euler-potential})
% and~(\ref{eq:incompressible-euler-perturbation-potential}) are
% representative examples) is a natural framework in which the physics
% of a fluid problem can be naturally described, the equations of
% motion for the free surface evolution are Lagrangian in nature.

% Our ultimate goal is to recover as accurately as possible the
% \emph{shape} of the free surface and the \emph{pressure distribution}
% on the ship hull. In both cases, the dynamic and kinematic boundary
% conditions~(\ref{eq:fsDynamicLag}) and~(\ref{eq:fsKinematicLag}) play
% a fundamental role, either as a direct evolution equation for the free
% surface potential and for its elevation, or as an indirect boundary
% condition needed to recover either the full potential gradient (the
% velocity) from the resolution of the mass conservation equation, or
% the pressure, from Bernoulli's equation.

% Already at this stage, it should be noted that both equations contain
% a transport term of the type $\vb\cdot\nablab a =
% (\Vb_{\stream}- \Vb_{\sys}+ \nablab\phi )\cdot \nablab a$, where
% $a$ is either $\phi$ or $\eta$. When the velocity
% $(\Vb_{\stream}- \Vb_{\sys})$ dominates over the
% perturbation potential gradient $\nablab\phi$, severe stability issues
% may arise in the numerical discretization, and special care is
% required.


Problem~(\ref{eq:incompressible-euler-perturbation-potential}) can be
rewritten in terms of ALE derivatives as

\begin{subequations}
  \label{eq:incompressible-euler-perturbation-potential-ALE}
  \begin{alignat}{2}
    % \label{eq:bernoulli-phi-ALE}
    % & \frac{\delta\phi}{\delta t} +(\vb-\wb)\cdot\nablab\phi = -gz +
    % \ab_{\stream}\cdot\xb +
    % \frac{1}{2}\left|\nablab\phi\right|^2 &-\frac{p-p_a}{\rho} \qquad \text{in } \Omega(t)\\
    \label{eq:incompressibility-potential-perturbation-phi-ALE}
    & \Delta \phi = 0 & \text{ in } \Omega(t)\\
    \label{eq:fsDynamicSemiLag}
    & \frac{\delta\phi}{\delta t} +(\vb-\wb)\cdot\nablab\phi= -g\eta
    + \ab_{\stream}\cdot\xb+ \frac{1}{2}|\nablab\phi|^2 & -
    \mu\phin \qquad \text{ on } \Gamma^w(t) \\
    &\phi(\xb, 0) = \phi_0(\xb) &\text{ on }
    \Gamma^w(0)\label{eq:initial-condition-phi-ALE} \\
    \label{eq:non-penetration-condition-hull-ALE}
    &\phin =
    \nb\cdot(\Vb_{\boat}-\Vb_{\stream}) & \text{ on }
    \Gamma^{h}(t)\\
    &\phin = 0 & \text{ on }
    \Gamma^b(t)\cup\Gamma^{ff}(t) \\
    \label{eq:condition-on-ALE-velocity}
    &\wb\cdot \nb = \vb\cdot \nb &\text{ on }
    \Gamma(t),
  \end{alignat}
\end{subequations}
where we notice that, whenever $\wb=\vb$, we recover a fully
Lagrangian formulation (the ALE motion is, in this case, following the
particles motion and $\delta/\delta t \equiv D/Dt$). Similarly, if the
domain is fixed, and we set $\wb=0$, we recover the classical Eulerian
formulation~(\ref{eq:incompressible-euler-perturbation-potential}) on
fixed domains, and $\delta/\delta t \equiv \Pa/\Pa t$.

If the free surface can be seen as the graph of a single valued
function $\eta(x,y,t)$ of the horizontal components $x$ and $y$, then
\begin{equation}
  \label{eq:definition-eta}
  \xb = (x,y, \eta(x,y,t)) \qquad \text{ on }\Gamma^w(t),
\end{equation}
and, for a material particle on the free surface, we have
\begin{equation}
  \label{eq:particle-eta}
  \plag(\xlag,t)\cdot\eb_z = \eta(\plag(\xlag, t),t),
\end{equation}
where we define $\eta(\xb,t) :=
\eta(\xb\cdot\eb_x,\xb\cdot\eb_y,t)$. Taking the time derivative of
Equation~(\ref{eq:particle-eta}) we get
\begin{equation*}
  \frac{\Pa \plag}{\Pa t}(\xlag,t)\cdot\eb_z = \frac{\Pa \eta}{\Pa
    t}(\plag(\xlag, t),t) + \frac{\Pa \plag }{\Pa t}(\xlag, t)\cdot
  \nablab \eta(\plag(\xlag, t),t)  \qquad \text{ on } \hat\Gamma^w,
\end{equation*}
that is, in Eulerian form:
\begin{equation}
  \label{eq:particle-veolocity-on-freesurface-eulerian}
  \vb_z = \frac{\Pa \eta }{\Pa
    t} +\vb\cdot \nablab \eta = \frac{D \eta}{D t}\qquad \text{ on } \Gamma^w(t),
\end{equation}
where $\Pa\eta/\Pa z \equiv 0$. Proceeding in the same way for the ALE
deformation and the ALE velocity of the domain, we get
\begin{equation}
  \label{eq:ale-veolocity-on-freesurface-eulerian}
  \wb_z = \frac{\Pa \eta}{\Pa
    t} +\wb\cdot \nablab \eta = \frac{\delta \eta}{\delta t}\qquad \text{ on } \Gamma^w(t).
\end{equation}
%
%
Isolating $\Pa \eta/\Pa t$ in
Equation~(\ref{eq:particle-veolocity-on-freesurface-eulerian}) and
substituting in
Equation~(\ref{eq:ale-veolocity-on-freesurface-eulerian}), we get an
alternative expression for
Condition~(\ref{eq:condition-on-ALE-velocity})\footnote{That
  conditions~(\ref{eq:condition-on-ALE-velocity})
  and~(\ref{eq:fsKinematicSemiLag}) are equivalent in this framework,
  comes immediately from the observation that, when $\Gamma^w(t)$ is the
  graph of the function $\eta(x,y,t)$, then the normal to the surface
  $\Gamma^w(t)$ itself is given by a vector proportional to
  $\eb_z-\nablab\eta$. Substituting in
  Equation~(\ref{eq:condition-on-ALE-velocity}) gives immediately
  Equation~(\ref{eq:fsKinematicSemiLag}).},
\begin{equation}
  \frac{\delta\eta}{\delta t} +(\vb-\wb)\cdot\nablab\eta =
    \vb\cdot \eb_z
    \qquad \text{ on }\Gamma^w(t),\label{eq:fsKinematicSemiLag}
\end{equation}
%
which is valid for nonbreaking waves in which $\eta(x,y,t)$ is
single-valued. 

Equation~(\ref{eq:fsKinematicSemiLag}) is the kinematic boundary
condition for the evolution of the unknown free surface elevation
$\eta(x,y,t)$ which is often found in the literature of
semi-Lagrangian methods for potential free surface
flows~\cite{beck1994,BeckCaoLee-1993-a,scorpioPhD}.

% If the domain $\Omega(t)$ changes with time, on the boundary
% $\Gamma(t)$, the ALE velocity $\wb(\xb,t)$ cannot be arbitrary, since
% the ALE motion is required to follow the motion of the boundary itself
% to preserve the shape of the domain $\Omega(t)$. This is expressed by
% the boundary condition~(\ref{eq:condition-on-ALE-velocity}), which
% constraints the normal component of the ALE velocity to be the same as
% the normal component of the fluid velocity, on the entire
% $\Gamma(t)$. By this condition, we deduce that arbitrary tangential
% velocity can be applied to the hull surface $\Gamma^h(t)$, and that
% the $z$ component of ALE velocity on $\Gamma^w(t)$, is necessarily
% equal to $\delta\eta/\delta t$, while its horizontal components can be
% arbitrary, i.e., 
% \begin{equation*}
%   \wb(\xb,t) = \left(u,v,\frac{\delta \eta}{\delta t}\right) \qquad \text{ on } \Gamma^w(t).
% \end{equation*}
% %
% This is easily seen by noting that the normal to the free surface is
% From~(\ref{eq:definition-eta}),
% and~(\ref{eq:condition-on-ALE-velocity}) we get
% \begin{equation*}
%   \wb_z-\wb\cdot\nablab\eta = \vb_z-\vb\cdot\nablab\eta,
% \end{equation*}
% in which we observe that in the scalar product $\wb\cdot\nablab\eta$
% there is no $\wb_z$ component, since $\nablab\eta\cdot \eb_z \equiv
% 0$. Plugging in the right hand side of
% Equation~(\ref{eq:fsKinematicSemiLag}), we get $\wb_z =
% \delta\eta/\delta t$, \emph{independently} on the $x$ and $y$
% components of $\wb$. 
Equation (\ref{eq:fsKinematicSemiLag}) is rather general, and is valid
for \emph{arbitrary} values of horizontal ALE velocities. Suitable
values of $\Vb_{\stream}$ and $\Vb_{\sys}$ can be plugged into the
velocity field $\vb = (\Vb_\stream-\Vb_\sys +\nablab\phi)$ to specify
them for the desired reference frame. For instance, setting
$\Vb_{\stream} = \Vb_{\sys} = 0$, and
$\wb=\left(0,0,\frac{\delta\eta}{\delta t}\right)$, one obtains

\begin{eqnarray*}
\frac{\delta\eta}{\delta t} &=& \frac{\Pa\phi}{\Pa z}+\nablab\eta\cdot\left(\wb -\nablab\phi\right)
                               = \frac{\Pa\phi}{\Pa z}-\frac{\Pa\phi}{\Pa x}\frac{\Pa\eta}{\Pa x}
                                 -\frac{\Pa\phi}{\Pa y}\frac{\Pa\eta}{\Pa y}
\label{eq:fsKinematicContento}\\
\frac{\delta\phi}{\delta t} &=& -g\eta +
\frac{1}{2}|\nablab\phi|^2 + \nablab\phi\cdot\left(\wb -\nablab\phi\right) 
                               =  -g\eta + \frac{\Pa\phi}{\Pa z}\frac{\delta\eta}{\delta t}
\label{eq:fsDynamicContento},
\end{eqnarray*}  
%
which are the semi-Lagrangian equations written in an earth fixed reference frame, and null stream velocity
used in \cite{KjelContJans-2011}.


In this work, we choose instead to solve the problem in a coordinate
system attached to the ship hull. We move the reference frame
according to the horizontal average velocity of the boat, that is we
set $\Vb_\sys = (\overline\Vb_\boat\cdot\eb_x)\eb_x =: -\Vb_\infty =
\left(-V_\infty,0,0\right)$ and we assume $\Vb_{\stream} = 0$. With
these values, Equations (\ref{eq:fsKinematicSemiLag}) and
(\ref{eq:fsDynamicSemiLag}) take the form

\begin{eqnarray}
\frac{\delta\eta}{\delta t} &=& \frac{\Pa\phi}{\Pa z}+\nablab\eta\cdot\left(\wb -\nablab\phi-\Vb_\infty\right)
\label{eq:fsKinematicBeck}\\
\frac{\delta\phi}{\delta t} &=& -g\eta +
\frac{1}{2}|\nablab\phi|^2 + \nablab\phi\cdot\left(\wb -\nablab\phi-\Vb_\infty\right)-\mu\phin,
\label{eq:fsDynamicBeck}
\end{eqnarray}  
%
which coincide with the ones proposed by Beck \emph{et al.}
\cite{BeckCaoLee-1993-a}, and in which the points on the free surface
move with an a priori arbitrary horizontal speed in the boat
reference frame.

\subsection{Boundary integral formulation}

While
Equation~(\ref{eq:incompressibility-potential-perturbation-phi-ALE})
is time dependent and defined in the entire domain $\Omega(t)$, we are
really only interested in its solution on the boundary $\Gamma(t)$, in
particular on the unknown free surface part of the boundary, and on
the ship hull, where we would like to recover the pressure
distribution by postprocessing Bernoulli's
equation~(\ref{eq:bernoulli}).

At any given time instant $\overline{t}$ we want to compute $\phi$
satisfying
%
\begin{subequations}
\label{eq:laplace-problem}
\begin{alignat}{2}
-\Delta\phi &= 0 & \text{in} \ \ \Omega(\overline{t}) \\
\phi &= \overline{\phi} & \text{on} \ \ \Gamma^{w}(\overline{t}) \\
\phin &= \overline\phin   & \qquad\text{on} \ \ \Gamma^{h}(\overline{t})\cup\Gamma^{b}(\overline{t})\cup \Gamma^{ff}(\overline{t})  
\end{alignat}
\end{subequations}
%
where $\overline{\phi}$ is the potential on the free surface at the
time $\overline{t}$, and $\overline\phin$ is
equal to zero on $\Gamma^b(\overline{t} )\cup\Gamma^{ff}(\overline{t}
)$ and to $\big(\Vb_\boat(\overline{t})-\Vb_\infty(\overline{t})\big)\cdot\nb$ on
$\Gamma^{h}(\overline{t} )$.

This is a purely spatial boundary value problem, in which time appears
only through boundary conditions and through the shape of the time
dependent domain.

The solution of this boundary value problem allows the computation of
the full potential gradient on the boundary $\Gamma(t)$, which is what
is required in the dynamic and kinematic boundary conditions to
advance the time evolution of both $\phi$ and $\eta$.

Using the second Green identity
\begin{equation*}
  \int_{\Omega}
  (-\Delta u)v\,dx + \int_{\partial\Omega} \frac{\partial u}{\partial
    n}v \d s
  = 
  \int_{\Omega}
  (-\Delta v)u\,dx + \int_{\partial\Omega} \frac{\partial v}{\partial
    n} u \d s,
\end{equation*}
a solution to system (\ref{eq:laplace-problem}) can be expressed in terms
of a boundary integral representation only, via convolutions with
fundamental solutions of the Laplace problem.

We call $G$ the \emph{free space Green's function}, i.e., the function
\begin{equation*}
G(\rb)  =  \frac{1}{4\pi |\rb|},
\end{equation*}
%      
which is the distributional solution of
\begin{equation} \label{eq:poissonGreen}
  \begin{split}
    &-\Delta G(\xb-\xb_0) = \delta(\xb_0) \qquad\qquad
     \text{ in } \Re^3\\
    &\lim_{|\xb|\to\infty} G(\xb-\xb_0) = 0,
  \end{split}
\end{equation} 
%
where $\delta(\xb_0)$ is the Dirac distribution centered in $\xb_0$.

If we select $\xb_0$ to be inside $\Omega(t)$, use the defining property
of the Dirac delta and the second Green identity, we obtain
\begin{multline*}
\phi(\xb_0,t) =
\int_{\Omega(t)}\left[-\left(\Delta G(\xb-\xb_0)\right) \phi(\xb,t)\right] \d\Omega  = \\
\int_{\Gamma(t)} \left[(\nablab\phi(\xb,t)\cdot\nb)G(\xb-\xb_0) -
(\nablab G(\xb-\xb_0)\cdot\nb)\phi(\xb,t)\right]\d\Gamma.
\end{multline*}

In the limit for $\xb_0$ touching the boundary $\Gamma(t)$, the
integral on the right hand side will have a singular argument, and
should be evualated according to the Cauchy principal value. This
process yields the so called \emph{Boundary Integral Equation} (BIE)
\begin{equation}
\label{eq:bie}
\alpha\phi  = 
\int_{\Gamma(t)} \left[\phin G -
\frac{\Pa G}{\Pa n}\phi\right]\d\Gamma \qquad
  \text{ on } \Gamma(t),
\end{equation}
%
where $\alpha(\xb,t)$ is the fraction of solid angle $4\pi$ with which
the domain $\Omega(t)$ is seen from $\xb$ and the gradient of the free
space Green's function is given by
\begin{equation*}
\nablab G(\rb)\cdot \nb  = 
-\frac{\rb\cdot\nb}{4\pi \left|\rb\right|^3}.
\end{equation*} 
%

The function $\alpha(\xb,t)$ can be computed by noting that the
constant function $1$ is a solution to the Laplace equation with zero
normal derivative, and therefore it must be
\begin{equation}
  \label{eq:computation-alpha}
  \alpha = -\int_{\Gamma(t)} \frac{\Pa G}{\Pa n} d\Gamma\qquad
  \text{ on } \Gamma(t),
\end{equation}
in the Cauchy principal value sense.

With Equation~(\ref{eq:bie}), the continuity equation has been
reformulated as a boundary integral equation of mixed type defined on
the moving boundary $\Gamma(t)$, where the main ingredients are the
perturbation potential $\phi(\xb,t)$ and its normal derivative
$\displaystyle\phin(\xb,t)$.

The domain deformation $\pb(\xb,t)$ on the free surface takes the form
\begin{equation}
  \label{eq:def-ale-motion-gamma}
  \pb(\xb,t) = (x,y,\eta(x,y,t)) \qquad \text{ on } \Gamma^w(t), 
\end{equation}
and one has to solve an additional boundary value problem to uniquely
determine the full ALE motion $\pale(\xale,t)$.

\subsection{Arbitrary Lagrangian Eulerian motion}
\label{sec:arbitr-lagr-euler}



When the arbitrary Lagrangian Eulerian formulation is used in the
finite element framework (see, for
example,~\cite{formaggia2009cardiovascular}), the restriction to the
boundary $\Gamma(t)$ of the deformation $\pale(\xale,t)$ is either
known, or entirely determined by the equations of motion. In this
case, an additional boundary value problem needs to be solved to
recover the domain deformation in the interior of $\Omega(t)$ starting
from the Dirichlet values on the boundary.

Our situation is slightly different, since only the \emph{normal}
component of the motion is given on the boundary $\Gamma(t)$, and we
are not really interested in finding a domain motion in the interior
of $\Omega(t)$.

In the dynamic and kinematic boundary conditions
(\ref{eq:fsKinematicBeck}) and~(\ref{eq:fsDynamicBeck}) we have the
freedom to choose an ALE motion arbitrarily, as long as the shape of
$\Gamma(t)$ is preserved. In analogy to what is done in the finite
element framework, we construct an additional boundary value problem
to determine uniquely $\pale(\xale,t)$.

A typical choice in the finite element framework is based on linear
elasticity theory, and requires the solution of an additional Laplace
problem on the coordinates $\pale(\xale,t)$, or, in some cases, a
bi-Laplacian. This procedure can be generalized to surfaces embedded
in three-dimensional space via the Laplace-Beltrami operator. 

The Laplace-Beltrami operator can be constructed from the surface
gradient $\nablab_s g(\xb,t)$, defined as
\begin{equation}
  \label{eq:surface-gradient}
    \nablab_s a(\xb,t)  := \nablab
    \overline{a}-(\nablab\overline{a}\cdot\nb)\nb, \qquad
    \forall \overline a \text{ s.t. } \overline a = a(\xb,t) \quad\text{ on }\Gamma(t),
\end{equation}
where $\overline{a}$ is an arbitrary smooth extension of $a(\xb,t)$ on
a tubular neighborhood of
$\Gamma(t)$. Definition~(\ref{eq:surface-gradient}) is independent on
the extension used (see, for example,
\cite{delfour2010shapes}). Similarly, we indicate with
$\tilde\nablab_s$ the surface gradient computed in the reference
domain $\tilde\Gamma$, with the same definition as
in~(\ref{eq:surface-gradient}), but replacing $\xb$ with $\xale$, and
performing all differential operators in terms of the independent
variable $\xale$ instead of $\xb$.

If we indicate with $\nablab_s\cdot$ the surface divergence (i.e., the
trace of the surface gradient $\nablab_s$), then the surface Laplacian
$\Delta_s$ and $\tilde\Delta_s$ on $\Gamma(t)$ and on $\tilde\Gamma$,
are given by $\Delta_s:= \nablab_s\cdot\nablab_s$, and by $\tilde\Delta_s:=
\tilde\nablab_s\cdot\tilde\nablab_s$.


We use the shorthand notation $\gamma^{a,b}(t)$
to indicate the intersection between $\Gamma^a(t)$ and $\Gamma^b(t)$,
that is,
\begin{equation*}
  \gamma^{a,b}(t) = \overline{\Gamma^a(t)}\cap \overline{\Gamma^b(t)}
  \qquad a \neq b,
\end{equation*}
where $a,b$ are either $w$, $h$, $b$ or $ff$. We indicate with
$\gamma(t)$ the union of all curves $\gamma^{a,b}(t)$. 

The curve $\gamma^{w,h}(t)$ is usually referred to as the
\emph{waterline} on the hull of the ship. On $\gamma^{w,h}(t)$, the
domain velocity $\wb$ has to satisfy the kinematic boundary condition
for \emph{both} the free surface and the ship hull:
\begin{equation}
  \label{eq:velocity-on-waterline}
  \begin{aligned}
    \wb\cdot\nb^w &= \vb\cdot\nb^w \qquad& \text{ on } \gamma^{w,h}(t)&\\
    \wb\cdot\nb^h &= 0 & \text{ on } \gamma^{w,h}(t)&,
  \end{aligned}
\end{equation}
where $\nb^w$ is the normal to the free surface and $\nb^h$ is the
normal to the hull surface. When both conditions are enforced, $\wb$
is still allowed to be arbitrary along the direction tangent to the
waterline. 

There are several options to select the tangent velocity $\wb_t$
defined as
\begin{equation*}
  \wb_t := \wb\cdot(\nb^h\times\nb^w) = \wb\cdot \tb.
\end{equation*}
%
A natural possibility is to choose zero tangential velocity. Other
choices are certainly possible, and may be preferable, for example, if
one would like to cluster computational nodes in regions where the
curvature of the waterline is higher. In the experiments we present,
the tangential velocity is always set to zero.

Conditions~(\ref{eq:velocity-on-waterline}) and zero tangential
velocity, uniquely determine an evolution equation for the ALE
deformation on $\tilde\gamma^{w,h}$. Here we summarize all boundary
conditions for the evolution of $\pale(\xale,t)$ on the entire
$\tilde\gamma$:
\begin{subequations}
  \label{eq:w-cond-gamma}
  \begin{align}
    \wb\cdot\nb^w &= \vb\cdot\nb^w \qquad& \text{ on } \gamma^{w,h}(t)&\nonumber\\
    \wb\cdot\nb^h &= 0 & \text{ on } \gamma^{w,h}(t)& \label{eq:w-cond-gamma-w-h}\\
    \wb\cdot(\nb^h\times\nb^w) &= 0 & \text{ on } \gamma^{w,h}(t)&\nonumber\\
    \nonumber\\
    \wb\cdot\nb^w &= \vb\cdot\nb^w \qquad& \text{ on } \gamma^{w,ff}(t)&\nonumber\\
    \wb\cdot\nb^{ff} &= 0 & \text{ on } \gamma^{w,ff}(t)& \label{eq:w-cond-gamma-w-ff}\\
    \wb\cdot(\nb^w\times\nb^{ff}) &= 0 & \text{ on } \gamma^{w,ff}(t)&\nonumber\\
    \nonumber\\
    \wb  &= 0 \qquad& \text{ on }
    \gamma^{b,ff}(t)&.\label{eq:w-cond-gamma-b-ff}
  \end{align}
\end{subequations}
%
Expressing the boundary conditions~(\ref{eq:w-cond-gamma}) as a given
velocity term $\wb_g$, the evolution equation of $\gamma(t)$ become
\begin{equation}
  \label{eq:evolution-gamma}
  \begin{aligned}
    \frac{\Pa\pale_\gamma}{\Pa t}(\xale,t) &= \wb_g(\pale_\gamma(\xale,t)) \qquad
    &\text{ on } \tilde\gamma&\\
    \pale_\gamma(\xale,0) &= \pale_0(\xale) \qquad &\text{ on } \tilde\gamma&.
  \end{aligned}
\end{equation}

A reconstruction of a reasonable ALE deformation on the entire
$\Gamma(t)$ is then possible by solving an additional elliptic
boundary value problem, coupled with a projection on the surface of
the ship hull and on the free surface. Given a free surface
configuration $\eta$ and the deformation $\pale_\gamma$ on the
wireframe $\tilde\gamma$, in order to find a compatible deformation
$\pale$ on the entire $\tilde\Gamma$, we solve the additional problem
\begin{equation}
  \label{eq:laplace-beltrami-on-Gamma}
  \begin{aligned}
    & -\tilde\Delta_s \tilde \gb = -2\tilde\nb \tilde k  \qquad & \text{ on }
    \tilde\Gamma&\\
    & \tilde \gb = \pale_\gamma  & \text{ on } \tilde\gamma&\\
    \\
    &\pale = \mathcal{P}_h\,\tilde \gb  \qquad
    & \text{ on } \tilde\Gamma^h&\\
    & \pale = \mathcal{P}_\eta \,\gale := \gale + (\eta(\gale)-\gale\cdot\eb_z)\eb_z 
    & \text{ on } \tilde\Gamma^w&\\
    \\
    & \pale = \gale 
    & \text{ on } \tilde\Gamma^b\cup\tilde\Gamma^{ff},
  \end{aligned}
\end{equation}
where $\tilde k(\xale)$ is the mean curvature of the domain $\tilde\Gamma$,
i.e., the mean curvature of the hull on $\tilde\Gamma^h$ and zero
eveywhere else, while $\mathcal{P}_h$ is a projection operator on the
hull surface. Similarly, $\mathcal P_\eta$ is a (vertical) projection
operator on the free surface. 

The auxiliary function $\gale$ represents a surface that follows the
waterline deformation $\pale_\gamma$. On the ship hull, it is a
perturbation of the shape of the hull while everywhere else it is a
minimal surface with boundary conditions imposed by $\pale_\gamma$. On
the free surface, only its $x$ and $y$ components are used to
determine $\pale$, while $\eta$ (which satisfies the kinematic
boundary conditions~(\ref{eq:fsKinematicSemiLag})) imposes the $z$
component.

\subsection{Integro-differential formulation}
\label{sec:integro-diff-form}

Putting everything together, the final integro-differential system is
given by the following problem:

Given initial conditions $\phi_0$ and $\eta_0$ on $\Gamma^w(0)$, and
$\pale_0$ on $\tilde\gamma$, for each time $t\in [0,T]$, find $\pale$,
$\phi$, $\phin$ that satisfy
\begin{subequations}
  \label{eq:continuous-problem}
  \begin{alignat}{2}
    \label{eq:continuous-bie}
    & \int_{\Gamma(t)} \frac{\Pa G}{\Pa n}\phi \d\Gamma-\phi\int_{\Gamma(t)} \frac{\Pa G}{\Pa n} \d\Gamma
    = \int_{\Gamma(t)} \phin G \d\Gamma  & \text{ on } \Gamma(t)\\
    \label{eq:continous-fsDynamicSemiLag}
    & \frac{\delta\phi}{\delta t} = V_\phi(\phi,\phi_n,\eta,\wb)& \qquad  \text{ on } \Gamma^w(t) \\
    &\frac{\delta\eta}{\delta t} = V_\eta(\phi, \phi_n,\eta,\wb)
    & \text{ on }\Gamma^w(t)\label{eq:continuous-fsKinematicSemiLag}\\
    & \phi(\xb, 0) = \phi_0(\xb) &\text{ on }
    \Gamma^w(0)\label{eq:continuous-initial-condition-phi-ALE} \\ 
    &\eta(\xb, 0) = \eta_0(\xb) &\text{ on }
    \Gamma^w(0)\label{eq:continuous-initial-condition-eta-ALE} \\
    \label{eq:continous-non-penetration-condition-hull-ALE}
    &\phin = \overline{\phin} & \text{ on } \Gamma^{N}(t) \\
    \label{eq:continuous-ALE-velocity-condition}
    &\wb\cdot\nb = 0 & \text{ on } \Gamma^{N}(t) \\
    &-\tilde\Delta_s\gale = -2\tilde\nb k \qquad &\text{ on }
    \tilde\Gamma\setminus\tilde\gamma\\
    &\frac{\Pa\gale_\gamma}{\Pa t}(\xale,t) = \wb_g(\gale(\xale,t)) \qquad
    &\text{ on } \tilde\gamma\\
    &\pale(\gale,0) = \pale_0(\gale) \qquad &\text{ on }
    \tilde\gamma&\\
    & \pale = \mathcal P\,\gale &\text{ on }
    \tilde\Gamma.
  \end{alignat}
\end{subequations}
where we used the shorthand notations
\begin{subequations}
  \begin{align}
    \wb &:= \frac{\delta \pb}{\delta t}\\
    \label{eq:def-total-V}
    \vb & := \Vb_\infty-\Vb_\sys+\nablab\phi\\
    \label{eq:def-V-phi}
    V_\phi(\phi,\phi_n,\eta,\wb) &:= (\wb-\vb)\cdot\nablab\phi-g\eta + \ab_{\infty}\cdot\xb+
    \frac{1}{2}|\nablab\phi|^2 -\mu\phin \\
    \label{eq:def-V-eta}
    V_\eta(\phi,\phi_n,\eta,\wb) &:= (\wb-\vb)\cdot\nablab\eta + \vb\cdot
    \eb_z \\
    \Gamma^N(t) &:= \Gamma^{h}(t)\cup\Gamma^{b}(t)\cup\Gamma^{ff}(t) \\
    \overline\phin &:=
    \begin{cases}
      (\Vb_\boat-\Vb_\sys)\cdot\nb & \text{ on } \Gamma^h(t) \\
      0 & \text{ on } \Gamma^{b}(t)\cup\Gamma^{ff}(t),
    \end{cases}\\
    \label{eq:projection-operator}
    \mathcal P \gale& :=
    \begin{cases}
      \mathcal{P}_h \,\gale  & \text{ on } \tilde\Gamma^h\\
      \mathcal{P}_\eta\, \gale:= \gale + (\eta(\gale,t)-\gale\cdot\eb_z)\eb_z 
       & \text{ on } \tilde\Gamma^w\\
      \gale  & \text{ on } \tilde\Gamma^b\cup \tilde\Gamma^{ff},
    \end{cases}
  \end{align}
\end{subequations}
and both the potential and the pressure in the entire domain can be
obtained by postprocessing the solution to
Problem~(\ref{eq:continuous-problem}) with the boundary integral
representation~(\ref{eq:poissonGreen}) and with Bernoulli's
Equation~(\ref{eq:bernoulli}). 

The full gradient of the perturbation potential on the surface
$\Gamma(t)$ that appears in Equations~(\ref{eq:def-total-V}),
(\ref{eq:def-V-phi}) and~(\ref{eq:def-V-eta}) is constructed from the
surface gradient of $\phi$ and from the normal gradient $\phin$ as
\begin{equation*}
  \nablab \phi(\xb,t) := \nablab_s\phi(\xb,t) +\phin(\xb,t)\nb.
\end{equation*}

A numerical discretization of the continuous
Problem~(\ref{eq:continuous-problem}) is done on the \emph{fixed}
boundary $\tilde\Gamma$ of the reference domain $\Oale$, with
independent variable $\xale$ which will label node locations in a
reference computational grid, and the motion $\pale(\xale,t)$ will
denote the trajectory of the computational nodes.

% We look for solutions $\displaystyle(\pb,\phi, \phin)$ of
% Problem~(\ref{eq:continuous-problem}) in the spaces $Y\times[0,T]$,
% $V\times[0,T]$ and $Q\times[0,T]$, where
% \begin{subequations}
%   \label{eq:continuous-spaces}
%   \begin{alignat}{5}
%     \label{eq:space-x} {Y} &:= \Bigl\{\ub \in
%     W^{1,\infty}(\tilde\Gamma)^3, \text{ s.t. } \exists \quad\ub^{-1}
%     \in W^{1,\infty}(\tilde\Gamma)^3&& \Bigr\}\\
%     \label{eq:space-phi-tilde}
%     {V} &:= \Bigl\{ \phi \in H^{\frac{1}{2}}(\tilde\Gamma) &&\Bigr\}\\
%     \label{eq:space-phin-tilde}
%     {Q} &:= \Bigl\{ \gamma \in H^{-\frac{1}{2}}(\tilde\Gamma)&& \Bigr\},
%   \end{alignat}
% \end{subequations}
% and all differential operators are transformed via a standard change
% of variables to the reference domain boundary $\tilde\Gamma$.


\section{Numerical discretization}
\label{sec:numer-discr}

To approximate the continuous problem, we introduce a decomposition
$\tilde\Gamma_{h}$ for $\tilde\Gamma$ made of quadrilaterals in three
dimensional space, such that the usual regularity assumptions are
satisfied:
%%
\begin{enumerate}
\item $\overline{\tilde\Gamma} = \cup \{ K \in \tilde\Gamma_{h} \}$;

\item
Any two cells $K,K'$ only intersect in common faces, edges, or vertices;

\item
The decompositions $\tilde\Gamma_{h}$ matches the decomposition
$\tilde\Gamma = \tilde\Gamma^w \cup \tilde\Gamma^h \cup\tilde\Gamma^b
\cup \tilde\Gamma^{ff}$.
\end{enumerate}
%%
On the decomposition $\tilde\Gamma_{h}$, we look for solutions
$\displaystyle(\pb_h,\phi_h, \phin_h)$ in the finite dimensional
spaces ${Y}_{h}$, ${V}_{h}$, and ${Q}_{h}$ defined as
%%
\begin{alignat}{5}
\label{eq:space-Y-h}
{Y}_{h} &:= \Bigl\{ \ub_h \in \mathcal{C}^0(\tilde\Gamma_h)^3 \,&&\big|\, \ub_{h|K} &&\in \mathcal{P}_Y(K)^3, \, K &&\in \tilde\Gamma_h \Bigr\} &&\equiv \vssp\{ \vb_{h}^{i} \}_{i=1}^{N_{Y}}\\
\label{eq:space-phi-h}
{V}_h &:= \Bigl\{ \phi_h \in \mathcal{C}^0(\tilde\Gamma_h)  \,&&\big|\, \phi_{h|K}  &&\in \mathcal{P}_V(K), \, K &&\in \tilde\Gamma_h \Bigr\} &&\equiv \vssp\{ \varphi_{h}^{i} \}_{i=1}^{N_{V}}
\\
\label{eq:space-phin-h}
{Q}_h &:= \Bigl\{ \gamma_h \in \mathcal{C}^0(\tilde\Gamma_h)  \,&&\big|\, \gamma_{h|K}  &&\in \mathcal{P}_Q(K), \, K &&\in \tilde\Gamma_h \Bigr\} &&\equiv \vssp\{ \tau_{h}^{i} \}_{i=1}^{N_{Q}},
\end{alignat}
%% 
where $\mathcal{P}_{Y}(K)$, $\mathcal{P}_{V}(K)$ and
$\mathcal{P}_{Q}(K)$ are polynomial spaces of degree $r_{Y}$, $r_{V}$
and $r_{Q}$ respectively on the cells $K$, and $N_Y$, $N_V$ and $N_Q$
are the dimensions of each finite dimensional space.

The most common approach for the solution of the boundary integral
equation~(\ref{eq:bie}) in the engineering community is the
\emph{collocation boundary element method}, where the continuous
functions $\phi$ and $\nablab \phi \cdot \nb$ are replaced by their
discrete counterparts and the boundary integral equation is imposed
at a sufficient number of points on $\Gamma(t)$.

Once a geometric representation of the reference domain
$\tilde\Gamma_h$ is available as a collection of quadrilaterals $K$,
we could in principle choose arbitrary discretizations of the
functional spaces $V_h$, $Q_h$ and $Y_h$, which may not be related
with the geometrical discretization. A more natural choice, however,
is given by the \emph{iso-parametric} representation, where the shape
of the deformed surface $\Gamma_h(t)$, i.e., the map $\pale(\xale,t)$,
the surface potential $\phi_h(\xb,t)$ and its normal derivative
$\displaystyle\phin(\xb,t)$ on the $k$-th panel are based on the same
parametrization used for the panel geometry, that is, we choose
\begin{equation}
  \label{eq:space-choice}
  Q_h = V_h, \qquad Y_h = V_h^3 = \vssp\{ \varphi_{h}^{i}\eb_x, 
  \varphi_{h}^{i}\eb_y,\varphi_{h}^{i}\eb_z \}_{i=1}^{N_{V}}.
\end{equation}
%
We indicate with the notation $\{\phi\}$ and
$\displaystyle\left\{\phin\right\}$ the column
vectors of time dependent coefficients $\phi^i(t)$ and
$\displaystyle\phin^j(t)$ such that
\begin{equation}
  \label{eq:coefficient-notation}
  \begin{split}
    \phi_h(\xb, t) & := \sum_{i=1}^{N_V}
    \phi^i(t)\varphi^i_h(\pale_h^{-1}(\xb,t)) \qquad\text{ on }\Gamma_h(t)\\
    \phin_h(\xb, t) &:= \sum_{j=1}^{N_V}
    \phin^j(t)\varphi^j_h(\pale_h^{-1}(\xb,t))  \qquad\text{ on }\Gamma_h(t),
  \end{split}
\end{equation}
where the map $\pale_h^{-1}(\xb,t)$ is the inverse of the ALE
deformation
\begin{equation}
  \label{eq:control-points}
  \pale_h(\xale, t) := \sum_{k=0}^{N_V}\xb^k(t)\varphi^k_h(\xale) \qquad\text{ on }\tilde\Gamma,
\end{equation}
and $\xb^k$ represents the current location of the vertices or
control points that define the current configuration of
$\Gamma(t)$. 

To distinguish matrices from column vectors, we will indicate matrices
with the bracket notation, e.g.., $[M]$. The ALE derivatives of the
finite dimensional $\phi_h(\xb,t)$ and $\pb_h(\xb,t)$ can be
expressed as
\begin{equation}
  \label{eq:ale-derivative-discrete}
  \begin{split}
    \frac{\delta \phi_h}{\delta t}(\xb, t) & = \sum_{i=1}^{N_V}
    \frac{\Pa
      \phi^i}{\Pa t}(t)\varphi^i_h(\pale_h^{-1}(\xb,t)) \\
    \wb_h(\xb, t) := \frac{\delta \pb_h}{\delta t}(\xb, t) & = \sum_{i=1}^{N_V} \frac{\Pa
      \xb^i}{\Pa t}(t)\varphi^i_h(\pale_h^{-1}(\xb,t)),
  \end{split}
\end{equation}
that is, they are time parametrized finite dimensional vectors in
$V_h$ and $Y_h$ identified by the coefficients $\{\phi\}'$ and by the
control points $\{\xb\}'$, where the $'$ denotes derivation in time.

We can reconstruct the full discrete gradient $\nablab\phi_h$ on
$\Gamma_h(t)$ using the discrete version of the surface gradient
$\nablab_s$ and the normal gradient $\phin_h$:
\begin{equation}
  \label{eq:surface-discrete-gradient}
  \begin{split}
    \nablab_s\phi_h(\xb, t) & := \sum_{i=1}^{N_V} \phi^i(t)
    \nablab_s\varphi^i_h(\pale_h^{-1}(\xb,t)) \qquad\text{ on
    }\Gamma_h(t)\\
    \nablab\phi_h(\xb, t) & = \nablab_s\phi_h(\xb, t) + \phin_h(\xb,t)\nb  \qquad\text{ on }\Gamma_h(t).
  \end{split}
\end{equation}

In general, the gradients defined in
Equation~(\ref{eq:surface-discrete-gradient}) are not necessarily
continuous across the edges of the elements $K$ which determine the
surface discretization $\Gamma_h(t)$, unless all the basis functions
of the space $V_h$ are globally of class $\mathcal C^1$. While this is
certainly a possibility, it is not strictly necessary to solve a
discrete version of Problem~(\ref{eq:continuous-problem}).


% \section{The continuous problem}
% \label{sec:cont_prob}

% Problem~(\ref{eq:continuous-problem}) can be recast in the following
% form

% \begin{equation}
% \label{eq:int_diff_formulation}
%   F(t, y, \dot{y}) = 0,
% \end{equation}
% where we grouped the variables of the system in the vector $y$,

% \begin{equation}
% y = \left\{\xb, \phi, \phi_n\right\}
% \end{equation}
% %
% which contains respectively the motion of the material points of the original domain boundary $\Pa\Omega$,
% the potential field and the potential normal derivative. The residual function $F$ reads

% \begin{equation}
% \label{eq:int_diff_residual}
% \left\{
% \begin{array}{l l l}
% x^{w} - S_x(\xb) &=& 0 \\
% y^{w} - S_y(\xb) &=& 0 \\
% \dot{\eta}^{w} - V_{\eta}(\xb,\phi,\phi_n) &=& 0 \\
% x^{b} - S_x(\xb) &=& 0 \\
% y^{b} - S_y(\xb) &=& 0 \\
% z^{b} - S_z(\xb) &=& 0 \\
% \dot{\phi}^{w} - V_{\phi}(\xb,\phi,\phi_n) &=& 0 \\
% \alpha\phi  - \int_{\Pa \Omega} \left[\phi_n G - G_n\phi\right]d\Gamma &=& 0,
% \end{array}
% \right .
% \end{equation} 

% where we made use of the following  


% One of the advantage of the boundary element method over volumetric
% approximation techniques, is given by the fact that the computational
% domain reduces to surfaces only, for which it is relatively simple to
% construct high quality discrete approximations.

\subsection{Iso-parametric discretization}
\label{sec:iso-param}

We approximate the geometry of the domain boundary by means of
arbitrary order quadrilateral panels, that is, panels for which the
sides and the interior are composed of polynomials and polynomial
tensor products respectively.

\begin{figure}[htb!]        
\centerline{\xfig[1]{pannello}}
\caption{A quadratic panel and the reference element \label{fig:panel}}	
\end{figure}  

In particular we define the Lagrangian shape functions $N_l(u,v) \quad
l = 1,\dots,N_L$ on the reference panel (on the left in
Fig. \ref{fig:panel} we present an example for the quadratic case),
which allow us to introduce a local parametrization of the $k$-th
panel as 
\begin{equation}
  \label{eq:local-gamma-h}
  \begin{split}
    \xale_k(u,v) &:= \sum_{l=1}^{N_L} \xale^{k_l} N_l(u,v) \qquad \qquad
    u,v\in[0,1]^2\\
    \xb_k(u,v,t) &:= \sum_{l=1}^{N_L} \xb^{k_l}(t) N_l(u,v) \qquad \qquad
    u,v\in[0,1]^2,
  \end{split}
\end{equation}
%
where the weights are the positions of the nodes in the reference
domain $\tilde\Gamma_h$, or the nodes in the current domain
$\Gamma_h(t)$, and $k_l$ is the \emph{local to global} numbering index
which identifies the $N_L$ basis functions $\varphi^{k_l}$ which are
different from zero on the $k$-th panel. The current geometry
$\Gamma_h(t)$ is constructed with $\xb^{k_l}(t)$ instead of
$\xale^{k_l}$, but with the same local parametrization, avoiding the
need to explicitly construct the inverse of the map $\pale(\xale,t)$,
since we rewrite everything in terms of local coordinates on each
single panel $K$.

The global basis functions $\varphi^i(\xale)$ can be identified
and evaluated on each panel $K$ via their local parametrization as
\begin{equation}
  \label{eq:global-basis}
  \varphi^i_k(u,v) := \varphi^i(\xale_k(u,v)) =  \sum_{l=1}^{N_L}\delta_{i\,k_l}N_l(u,v),\qquad 
  \delta_{ij} =
  \begin{cases}
    1 & \text{ if } i = j\\
    0 & \text{ otherwise.}
  \end{cases}
\end{equation}

At this point, a local representation of $\phi(\xb^k(u,v,t),t)$ and of
its normal derivative on the $k$-th panel are available as
\begin{equation*}
\phi_k(u,v,t) = \sum_{l=1}^{N_L} \phi^{k_l}(t) N_l(u,v) \qquad
\phin{}_k(u,v,t) =
\sum_{l=1}^{N} \phin ^{k_l}(t)
N_l(u,v),
\end{equation*}
%
where $\phi^{k_l}, \phin^{k_l}
\,\,l=1,\dots,N_L$ are the nodal values of the potential and of its
normal derivative in panel $k$.  

There are arguments in favor of selecting a different representation
for $\phin$, based on the consideration that the
normals are, in general, not continuous across neighboring panels, but
a very reasonable approximation can be obtained, provided that the
discontinuities are taken into account where the domain of integration
presents sharp features, like corners or edges. In this work, we employ
a technique for the treatment of edges and corners developed by Grilli and
Svendsen (\cite{grilliCorner90}).

%
On each point of the panel, it is possible to compute two vectors
tangential to $\Gamma_h(t)$ as
\begin{equation*}
\tb_u^k(u,v,t) = \sum_{l=1}^{N_L} \xb^{k_l}(t) \frac{\Pa N_l}{\Pa u}(u,v)
\qquad
\tb_v^k(u,v,t) = \sum_{l=1}^{N_L} \xb^{k_l}(t) \frac{\Pa N_l}{\Pa v}(u,v),
\end{equation*}
%
%\begin{equation*}
%\tb_u^k(u,v) = \frac{\sum_{i=1}^{8} \xb_i^k \frac{\Pa N_i}{\Pa u}(u,v)}
%{\left|\left|\sum_{i=1}^{8} \xb_i^k \frac{\Pa N_i}{\Pa u}(u,v)\right|\right|_2}
%\qquad
%\tb_v^k(u,v) = \frac{\sum_{i=1}^{8} \xb_i^k \frac{\Pa N_i}{\Pa v}(u,v)}
%{\left|\left|\sum_{i=1}^{8} \xb_i^k \frac{\Pa N_i}{\Pa v}(u,v)\right|\right|_2},
%\end{equation*}
from which the external normal unit vector $\nb$ is obtained as
\begin{equation} \label{eq:normalComp}
\nb_{vect}^k(u,v,t) = \tb_u^k(u,v,t) \times \tb_v^k(u,v,t),
\qquad
\nb^k(u,v,t) = \frac{\nb_{vect}^k(u,v,t)}
                    {\left|\nb_{vect}^k(u,v,t)\right|}.
\end{equation}

The same can be done for vectors tangential and normal to
$\tilde\Gamma$, by simply replacing $\xb^{k_l}(t)$ with $\xale^{k_l}$
in the definitions above. We will denote those vectors with
$\tilde\tb_u^k(u,v)$, $\tilde\tb_v^k(u,v)$, $\tilde\nb_{vect}^k(u,v)$
and $\tilde\nb^k(u,v)$, respectively.

Integrals on a panel $K$ (or $\tilde K$), can be computed in the
reference domain $[0,1]^2$, by observing that $\d \Gamma = J^k(u,v,t)
\d u\d v$, where $J^k(u,v,t):=|\nb_{vect}^k(u,v,t)|$ (or $\d
\tilde\Gamma = \tilde J^k(u,v) \d u\d v$, where $\tilde
J^k(u,v):=|\tilde\nb_{vect}^k(u,v)|$).

Denoting with
\begin{equation*}
  \begin{split}
    D_k(u,v,t) &:= \nablab_{uv} \xb_k(u,v,t)
    \qquad\in\Re^{3\times2}\\
    G_k(u,v,t) &:= D_k(u,v,t)^T
    D_k(u,v,t)\qquad \in\Re^{2\times2}\\
    \tilde D_k(u,v) &:= \nablab_{uv} \xale_k(u,v)
    \qquad\in\Re^{3\times2}\\
    \tilde G_k(u,v) &:= \tilde D_k(u,v)^T
    \tilde D_k(u,v)\qquad \in\Re^{2\times2},
  \end{split}
\end{equation*}
where $D_k$ and $\tilde D_k$ are the first fundamental forms in the
element $K$ and $\tilde K$, we can express locally the surface
gradient $\nablab_s$ (respectively $\tilde\nablab_s$) of the basis
functions on $K$ (respectively on $\tilde K$) as
\begin{equation}
  \label{eq:local-surface-gradient-basis-functions}
  \begin{split}
    \left.\nablab_s\varphi^i(\pale^{-1}(\xb,t))\right.|_{\xb=\xb_k(u,v,t)}
    & = D_k(G_k)^{-1} \nabla_{uv} \varphi^i_k(u,v,t) \\
    & =: \nablab_s  \varphi^i_k(u,v,t)\\
    \left.\tilde\nablab_s\varphi^i(\xale)\right.|_{\xale=\xale_k(u,v)}
    & = \tilde D_k(G_k)^{-1} \nabla_{uv} \varphi^i_k(u,v) \\
    & =: \tilde \nablab_s  \varphi^i_k(u,v),
  \end{split}
\end{equation}
which we will indicate with the same symbol as the spatial surface
gradients. The surface gradient of a finite dimensional vector can then
be computed by Equation~(\ref{eq:surface-discrete-gradient}).

%
%

\subsection{Collocation boundary element method}
\label{sec:collocation-bem}



With the iso-parametric representation, the discrete version of the
BIE, written for an arbitrary point $\yb$ on the domain boundary, can
be decomposed using the local contributions of the $N_L$ basis functions
in each of the $M$ panels of the triangulation:
\begin{multline}
    \alpha(\yb,t)\phi(\yb,t)  = \\
    -\sum_{k=1}^{M}\sum_{i=1}^{N_V} \phi^i(t)
    \int_{\hat K} \frac{\Pa G}{\Pa n}(\yb-\xb^k(u,v,t))
    \varphi^i_k(u,v)  J^k(u,v,t) \d u \d v \\
    + \sum_{k=1}^{M}\sum_{i=1}^{N_V} \left(\frac{\Pa \phi}{\Pa
        n}(t)\right)^i \int_{\hat K} G(\yb-\xb^k(u,v,t))  \varphi^i_k(u,v)  J^k(u,v,t) \d
    u \d v.
\label{eq:discBIE1}
\end{multline}
% 

The numerical evaluation of the panel integrals appearing in equation
(\ref{eq:discBIE1}) needs some special treatment, due to the presence
of the singular kernels $G(\yb-\xb)$ and $\frac{\Pa G}{\Pa
  n}(\yb-\xb)$. Whenever $\yb$ is not a node of the integration panel,
the integral argument is not singular, and standard Gauss quadrature
formulas can be used. If $\yb$ is a node of the integration panel, the
integral kernel is singular and special quadrature rules are used,
which remove the singularity by performing an additional change of
variables (see, for example, \cite{lachatWatson}). In the framework of
collocated BEM, an alternative possibility would have been represented by
desingularized methods, in which the fundamental solutions are centered
at points that are different from the evaluation points. Typically, this
is obtained by centering the Green's functions at points that are
slightly outside the domain. Although these methods avoid dealing with
singular integrals, they pose problems on establishing a general rule
for suitable positioning of the fundamental solutions centers.
In the case at hand, the domain presents sharp edges and narrow corners
(typically found the bow or stern of a hull) which make the latter
task nontrivial.

 
% We describe it by considering the case where the singularity point
% $\Pb$ coincides with node 1 in the panel. If we split the panel into
% two triangular parts divided by the panel diagonal, the Jacobian of
% the transformation from the reference panel to one of the two
% triangular parts contains a term which is proportional to $R$. We can
% then use two standard Gauss quadrature rules, collapsed on the two
% triangles. For the lower triangle $T_L$, for example, the
% transformation can be written explicitly as
% \begin{equation}
%   \label{eq:singular-quad-mapping}
%   \begin{aligned}
%     F_L: (0,1)^2 & \mapsto T_L \\
%     (u^{SG},v^{SG}) & \mapsto \left(u^{SG}, u^{SG} \tan\left(\frac{\pi v^{SG}}{4}\right)\right),
%   \end{aligned}
% \end{equation}
% which is illustrated in Fig.~\ref{fig:quadSingKer}.  
% The Jacobian of the tranformation $F_L$ is given by
% \begin{equation}
%   \label{eq:jacobian-FL}
%   J_{F_L} = \frac{\pi \sqrt{u^2+v^2} }{4 \cos(\pi/4 v)},
% \end{equation}
% which contains a term that will remove the singularity $1/R$ upon
% integration. The additional transformation doubles the cost of
% integration on the singular elements. An equivalent transformation is
% made for the upper triangle, and combinations of several
% transformations like this one can be devised for integration on panels
% where the singularity is on arbitrary points inside the panel, or on a
% edge of the panel (for a complete treatment of these transformations,
% see, e.g.,~\cite{lachatWatson,erichsen1998efficient}).

% The resulting quadrature nodes and weights on the reference element
% are shown in green in Fig.~\ref{fig:quadSingKerNum}. The red nodes are
% instead obtained when the upper triangular part of the panel is
% considered.

% \begin{figure}[htb!]
% \centerline{\xfig[1]{quadratura}}       	
% \caption{The quadrature nodes for singular kernel \label{fig:quadSingKer}}
% \end{figure}

% \begin{figure}[htb!]

% \begin{center}
% \includegraphics[width=0.4\textwidth]{figures/quadNodes}       	
% \caption{The quadrature nodes for singular kernel \label{fig:quadSingKerNum}}
% \end{center}
% \end{figure}

If we write the boundary integral equation for each support point
$\xb^i$, $i=1,\dots,N_V$, we can finally recast the discrete version
of the boundary integral equation as
	
\begin{equation}
\label{eq:solvingSysFMM}
\left[\alpha\right]\left\{\phi\right\} + \left[N\right]\left\{\phi\right\} =
\left[D\right]\left\{\phin\right\}
\end{equation}
%
where we have used the following notation
	
\begin{itemize}
	
\item $\left\{\phi\right\}$ and $\left\{\phin\right\}$
  are the vectors containing the potential and its normal
  derivative node values, respectively;
  
\item $\left[\alpha\right]$ is a diagonal matrix composed by the
  $\alpha(\xb_i(t))$ coefficients;
  
\item $\left[D\right]$ and $\left[N\right]$ are the Dirichlet and
  Neumann matrices respectively whose elements are
%	
\begin{eqnarray*}
D_{ij} &=& \sum_{k=1}^{M}
                       \int_{\hat K}
		       G(\xb_i(t)-\xb^k(u,v,t))
                       \varphi^j_k(u,v)J^k(u,v,t) \d u \d v \\
N_{ij} &=& \sum_{k=1}^{M}
                       \int_{\hat K}
		       \frac{\Pa G}{\Pa n}(\xb_i(t)-\xb(u,v,t))
		         \varphi^j_k(u,v)J^k(u,v,t) \d u \d v. \\
\end{eqnarray*}
\end{itemize}	

The evaluation of the nodal values for the solid angle fractions
$\alpha_i$ appearing in the BIE equation is obtained considering the
solution to Laplace problem~(\ref{eq:laplace-problem}) when
$\phi\equiv 1$ in $\Omega(t)$. In this case, system
(\ref{eq:solvingSysFMM}) reads

\begin{equation*}  
\left[\alpha\right]\left\{1\right\} +
\left[N\right]\left\{1\right\} = 0,
\end{equation*}
%
which implies
%
\begin{equation} \label{eq:rigidModes} 
\alpha_i = -\sum_{j=1}^{N} N_{ij} \qquad i = 1,\dots,N.
\end{equation}
%

% Introducing the boundary conditions we get a linear system whose
% solution is the approximated potential and potential normal
% derivatives on the whole domain boundary.

% We first perform the splitting
% %
% \begin{equation*}
% \{\phi\} = \{\overline{\phi}\}_D + \{\phi\}_N \qquad
% \left\{\phin\right\} =
% \left\{\phin\right\}_D +
% \left\{\overline{\phin}\right\}_N,
% \end{equation*}
% %
% where
% %
% \begin{subequations} \label{eq:vectDefine}
% \begin{equation}
% \overline{\phi}_{iD} = \left\{ \begin{array}{c}
%       \overline{\phi}_i \quad \xb_i \in \Gamma^D \\[2mm]
%       0 \quad \xb_i \in \Gamma^N
%       \end{array} \right.
% \qquad
% \phi_{iN} = \left\{ \begin{array}{c}
%       0 \quad \xb_i \in \Gamma^D \\[2mm]
%       \phi_i \quad \xb_i \in \Gamma^N
%       \end{array} \right.
% \end{equation}
% %
% and
% \begin{equation}
% \phin_{iN} = \left\{ \begin{array}{c}
%       \phin_i \quad \xb_i \in \Gamma^D \\[4mm]
%       0 \quad \xb_i \in \Gamma^N
%       \end{array} \right.
% \qquad
% \overline{\phin}_{iD} = \left\{ \begin{array}{c}
%       0 \quad \xb_i \in \Gamma^D \\[4mm]
%       \overline{\phin}_i \quad \xb_i \in \Gamma^N.
%       \end{array} \right. 
% \end{equation}	
% \end{subequations}
% %
% Here, the overline symbol indicates known values, prescribed by imposing
% the known boundary conditions, while $\Gamma^D$ and
% $\Gamma^N$ are the Dirichlet and Neumann
% portions of the domain boundary, respectively. The final form of the linear
% problem to be solved reads

% \begin{equation}  \label{eq:solvingSysFMM}
% \left[\alpha\right]\left\{\phi\right\}_N +
% \left[N\right]\left\{\phi\right\}_N -
% \left[D\right]\left\{\phin\right\}_D =
% \left[D\right]\left\{\overline{\phin}\right\}_N -
% \left[\alpha\right]\left\{\overline{\phi}\right\}_D -
% \left[N\right]\left\{\overline{\phi}\right\}_D,
% \end{equation}
% %
% which can be recast in the more familiar form

% \begin{equation} \label{eq:solvingSys}
% \left[A\right]\left\{u\right\} = \left\{b\right\},
% \end{equation}
% %
% where

% \begin{equation*}
% \left\{u\right\} = \left\{\phi\right\}_N +
% \left\{\phin\right\}_D,
% \qquad
% \left\{b\right\} = 
% \left[D\right]\left\{\overline{\phin}\right\}_N -
% \left[\alpha\right]\left\{\overline{\phi}\right\}_D -
% \left[N\right]\left\{\overline{\phi}\right\}_D,
% \end{equation*}
% %
% and where $[A]$ is defined by

% \begin{equation*}
% A_{ij} = \left\{ \begin{array}{c c}
%              \alpha_{j}\delta_{ij} + N_{ij} & \xb_j \in \Gamma^N \\
% 	     D_{ij} & \xb_j \in \Gamma^D.   
%             \end{array}\right.
% \end{equation*}

% The boundary element discretization method here described presents several
% advantages with respect to a classical finite elements method. 
% Only the boundary of the fluid domain needs to be discretized, thus reducing
% the number of the degrees of freedom of the solution system. In addition,
% the mesh generation complexity is highly reduced, as surface meshes are sensibly
% simpler to obtain than volume ones. For this reason, both the human and CPU
% time necessary to obtain a suitable mesh are reduced.
% Finally, the mesh and solution files dimensions associated with this kind of
% approach are orders of magnitude lower than the corresponding FEM files,
% allowing quicker handling and processing, and less mass memory requirements. 

% On the other hand, the main drawback of this method is given by the fact that
% both $\left[D\right]$ and $\left[N\right]$ are full: this
% means that the memory needed to store them is $\mathcal{O}(N^2)$. This
% compares unfortunately with the FEM where the matrices are sparse and their
% dimension grows linearly with the number of degrees of freedom.
	
%To overcome this problem, one can choose to employ an
%iterative algorithm such as GMRES ($\left[D\right]$ and $\left[N\right]$ are
%also non symmetric) that does not require to evaluate the matrix explicitly,
%but only its action on a given vector. Adopting such
%an approach, the memory requirement drops to $\mathcal{O}(N)$, at the price of
%the higher computational cost linked to the fact that we do not precompute the
%matrices entries.
	
%Nevertheless, the evaluation of all the integral kernels in
%equations (\ref{eq:kernels}) requires an amount of operations which is
%$\mathcal{O}(N^2)$. In facts, this problem is similar to the so called
%\emph{N-body problem}, where the electrostatic or gravitational forces
%exerted by a set of $N$ charges or masses are evaluated in $N$ points.

% The computational cost for this kind of problems can be significantly
% decreased to $\mathcal{O}(N)$, by applying
% a \emph{Fast Multipole Algorithm}. This methodology, based on the
% approximation of the reciprocal distances between the charges or masses
% by means of harmonic series, was originally developed by L.F. Greengard
% and V. Rokhlin in 1987 \cite{greengRokh} for the fast evaluation of
% potential fields in particle systems.

%In the next sections, the basic concepts of the Fast Multipole Method, and the
%details of its application to the Boundary Element Method will be briefly
%outlined.  

%\subsection{The rigid modes technique}


% \subsection{Edge treatment}


% In correspondence with an edge of the domain boundary, two contiguous
% elements of the mesh share one of their sides, on which the direction of the
% surface normal presents a discontinuity. In particular, the
% normal unit vectors on the nodes of the edge shared by two different
% panels will assume two different values, as depicted in Fig. \ref{fig:edge}.


% \begin{figure}[htb!]        
% \centerline{\xfig[.5]{edgesTreat}}
% \caption{The two different normal unit vectors of a node placed on  
%          an edge \label{fig:edge}}	
% \end{figure}

% The potential normal derivative
% $\left\{\phin\right\} = \nablab\phi\cdot\nb$ on such
% nodes will present two different values. For this reason, when a singled
% valued normal derivative for the potential on each edge node is imposed, the
% numerical problem becomes ill posed.
  
% To deal with the presence of sharp edges, we first prepare the mesh file so that
% each edge separates two different boundary condition zones. Then, each node on
% an edge can be readily identified as a node shared by two surface elements
% belonging to different boundary condition zones. At this point, each edge
% node shared by two surface elements is duplicated, so that two distinct nodes
% are present in the mesh, each belonging to one of the two elements on the edge. 
% At the considered location, the mesh will now contain two different nodes,
% each having a different normal unit vector. In this way, the number of degrees
% of freedom of the system has been increased so as to allow discontinuous
% values for the normal derivative of the potential.

% On the other hand, due to our choice of duplicating edge nodes, also the
% potential values on couples of duplicate nodes will in principle be different.
% A new set of equations is then introduced in the system, to impose the
% continuity of the potential on the edges. In other words, as we increased the
% number of the degrees of freedom to account for non continuous potential
% normal derivative at the edge nodes, we have to provide an additional number of
% equations to be able to solve the linear system: such equations are obtained by
% imposing the continuity of the potential on the duplicate nodes, namely

% \begin{eqnarray*}
% \phi(\xb_{i2}) &=& \overline{\phi(\xb_{i1})} \qquad \text{if}
% \quad \xb_{i1} \in \Gamma^D, \\
% \phi(\xb_{i2}) &=& \phi(\xb_{i1}) \qquad \text{if}
% \quad \xb_{i1} \in \Gamma^N, \\
% \end{eqnarray*}

% where $\xb_{i1}$ and $\xb_{i2}$ respectively indicate the original node and
% its duplicate. 

% %In the implementation these conditions are applied directly on the
% %matrix-vector products. If the original node is a Dirichlet node the
% %components of the left and right hand side vectors corresponding to the 
% %duplicate node are respectively set to

% %\begin{equation*}
% %\phi(\xb_{i2})
% %\qquad \text{and} \qquad
% %\overline{\phi(\xb_{i1})},
% %\end{equation*}
% %   
% %while, if the original node is a Neumann node we set the components of the
% %left and right hand side vectors corresponding to the duplicate nodes to

% %\begin{equation*}
% %\phi(\xb_{i2}) - \phi(\xb_{i1})
% %\qquad \text{and} \qquad
% %0
% %\end{equation*}
% %
% %respectively.

% \subsection{The discretized problem}
% \label{sec:discretized-problem}

\subsection{SUPG stabilization}
\label{sec:semi-discrete}



For the time evolution of the dynamic and kinematic boundary
conditions~(\ref{eq:continous-fsDynamicSemiLag})
and~(\ref{eq:continuous-fsKinematicSemiLag}), we need to evaluate the
surface gradient of the basis functions that appear in
Equation~(\ref{eq:surface-discrete-gradient}).

The gradient of the perturbation potential is not, in general,
continuous across the edges of the panels that compose $\Gamma_h(t)$,
and therefore it is not possible to write directly an evolution
equation for the vertices of the triangulation and for the potential
nodal values, since on the location of the nodes the forcing term is
not single valued.

It is certainly possible to solve this issue by using smooth finite
dimensional spaces, as in~\cite{grilli2001}, but this is not strictly
necessary. A possible alternative is to impose the evolutionary
boundary conditions via an $L^2$ projection in the $V_h$ space, i.e.,
we substitute Equations~(\ref{eq:continous-fsDynamicSemiLag})
and~(\ref{eq:continuous-fsKinematicSemiLag}) with
\begin{subequations}
  \label{eq:l2projection}
  \begin{alignat}{2}
     & \left(\frac{\delta\phi}{\delta t},
       \varphi\right)_w = \left(V_\phi, \varphi\right)_w\qquad
     &\forall \varphi \in V_h \label{eq:continuous-fsDinamicSemiLag-weak}\\
     &\left(\frac{\delta\eta}{\delta t},\varphi\right)_w = \big(V_\eta,\varphi\big)_w
     &  \forall \varphi \in V_h \label{eq:continuous-fsKinematicSemiLag-weak},
  \end{alignat}
\end{subequations}
where 
\begin{equation}
  \begin{split}
    \left(a,b\right)_w &= \int_{\Gamma^w(t)}ab\ \d\Gamma\\
    \left(a,b\right) &= \int_{\Gamma(t)}ab\ \d\Gamma.
  \end{split}
\end{equation}


\begin{figure}[htb!]
\begin{center}
\includegraphics[width=\textwidth]{./figures/sawTooth}
\end{center}
\caption{An example of the sawtooth instability developing on the
         stern of the hull without stabilization.
         \label{fig:sawtooth}}
\end{figure}

However, the forcing terms of the evolution
equations~(\ref{eq:def-V-phi}) and~(\ref{eq:def-V-eta}) contain a
transport term, respectively $\nablab\eta\cdot\left(\wb
  -\nablab\phi-\Vb_\infty+\Vb_\sys\right)$ and
$\nablab\phi\cdot\left(\wb -\nablab\phi-\Vb_\infty+\Vb_\sys\right)$,
which becomes dominant whenever $(\Vb_\sys-\Vb_\infty)$ is very
different from $\nablab\phi$, causing a sawtooth numerical instability
which in most cases develops in proximity of the hull stern, with
consequent blow up of the simulations (an example of such instability
is given in Figure~\ref{fig:sawtooth}).

%The instability can be attributed to the observed instabilities.% Such
% instability causes a severe deformation of the computational grid
% which results in poor approximations of nodal values of $\eta$ and
% $\phi$ gradients, eventually leading to numerical break down.

Once the $L^2$ projection machinery is in place, as in
Eq.~(\ref{eq:l2projection}), a natural and consistent stabilization
mechanism that reduces the observed instabilities is the Streamwise
Upwind Petrov--Galerkin (SUPG) scheme (see, for
example,~\cite{hughes1979,tezduyar2003computation}).  In the SUPG
framework, the plain $L^2$ projection in
system~(\ref{eq:l2projection}) is replaced by the weighted projection
\begin{subequations}
  \label{eq:supgl2projection}
  \begin{alignat}{2}
    & \left(\frac{\delta\phi}{\delta t},
      \varphi+\db\cdot\nablab_s\varphi\right)_w = \left(V_\phi,
      \varphi+\db\cdot\nablab_s\varphi\right)_w\qquad
    &\forall \varphi \in V_h \label{eq:continuous-fsDinamicSemiLag-weak-supg}\\
    &\left(\frac{\delta\eta}{\delta
        t},\varphi+\db\cdot\nablab_s\varphi\right)_w =
    \left(V_\eta,\varphi+\db\cdot\nablab_s\varphi\right)_w & \forall
    \varphi \in V_h\label{eq:continuous-fsKinematicSemiLag-weak-supg},
  \end{alignat}
\end{subequations}
where 
\begin{equation}
  \label{eq:definition-db}
  \db := \tau \left(\frac{\vb-\wb}{|\vb-\wb|}\right),
\end{equation}
and $\tau$ is a positive stabilization parameter which involves a
measure of the local length scale (i.e. the ``element length'') and
the local Reynolds and Courant numbers. Element lengths and
stabilization parameters were proposed for the SUPG formulation of
incompressible and compressible flows in~\cite{hughes1979}, and an in
depth study of the stabilization properties for free boundary problems
was presented in~\cite{tezduyar2003computation}, however, to the best
of the authors' knowledge, this is the first time that such
stabilization technique is applied directly to a boundary value
problem defined on a curved surface.

Expressing everything in terms of the basis functions for finite
dimensional space $V_h$, we get
\begin{subequations}
  \begin{align}
    &[M][P_{\Gamma^w}]\{\phi\}' = [P_{\Gamma^w}]\{V_\phi\} \\
    &[M][P_{\Gamma^w}]\{\eta\}' = [P_{\Gamma^w}]\{V_\eta\},
  \end{align}
\end{subequations}
where
\begin{subequations}
\begin{align}
M^{ij} := &
\left(\varphi^j,\varphi^i+\db\cdot\nablab_s\varphi^i\right) \nonumber\\
 = &\sum_{k=1}^{M}
\int_{\hat K}
\varphi^j_k(u,v)\big(\varphi^i(u,v)+\db\cdot\nablab_s\varphi^i(u,v)\big)J^k(u,v,t)
\d u \d v\\
P_{A}^{ij} := &
\begin{cases}
  \delta_{ij} & \text{ if } \xb^i(t) \in A(t) \\
  0 & \text{ otherwise}
\end{cases}\\
V_\phi^i := & \left(V_\phi,\varphi^i+\db\cdot\nablab_s\varphi^i\right)
\nonumber\\
= & \sum_{k=1}^{M}
\int_{\hat K}
V_\phi(u,v)\big(\varphi^i(u,v)+\db\cdot\nablab_s\varphi^i(u,v)\big)J^k(u,v,t)
\d u \d v\\
V_\eta^i := & \left(V_\eta,\varphi^i+\db\cdot\nablab_s\varphi^i\right)
\nonumber\\
= & \sum_{k=1}^{M}
\int_{\hat K}
V_\eta(u,v)\big(\varphi^i(u,v)+\db\cdot\nablab_s\varphi^i(u,v)\big)J^k(u,v,t) \d u \d v.
\end{align}
\end{subequations}


\subsection{Semi-discrete smoothing operator}

The semi-discrete version of the smoothing
problem~(\ref{eq:laplace-beltrami-on-Gamma}) can be obtained with a
finite element implementation of the scalar Laplace-Beltrami operator,
and its application to the different components of $\pale$.

A weak form of the Laplace-Beltrami operator on $\tilde\Gamma$ of a
scalar function $u$ in $V$ with Dirichlet boundary conditions $u_g$ on
$\tilde\gamma$ and forcing term $f$ is given by
\begin{equation}
  \label{eq:weak-laplace-beltrami} 
  \begin{aligned}
    &\left(\tilde\nablab_s u,
      \tilde\nablab_s\varphi\right)_{\tilde\Gamma} = \left(f,
      \varphi\right)_{\tilde\Gamma}  \qquad &\forall
    \varphi \in V_0\\
    & u = u_g \qquad& \text{ on } \tilde\gamma,
  \end{aligned}
\end{equation}
where we indicate with $V_0$ the space of functions $\varphi$ in $V$
such that their trace on $\tilde\gamma$ is zero (see, for example,
\cite{BonitoNochettoPauletti-2010-a} and the references therein for
some details on the numerical implementation of the Laplace-Beltrami
operator). 

The semi-discrete form of Equation~(\ref{eq:weak-laplace-beltrami})
can be written as
\begin{equation}
  [K]\{u\} = \{F\}, \label{eq:semidiscrete-laplace-beltrami}
\end{equation}
where
\begin{equation}
  \begin{aligned}
    K^{ij} := &
    \left(\tilde\nablab_s\varphi_h^j,\tilde\nablab_s\varphi_h^i\right) \\
    = &\sum_{k=1}^{M} \int_{\hat K} \tilde\nablab_s\varphi_k^j(u,v)
    \cdot \tilde
    \nablab_s \varphi_k^i(u,v) \tilde J_k(u,v) \d u \d v\\
    F^{i} := &
    \left(f,\varphi_h^i\right) \\
    = &\sum_{k=1}^{M} \int_{\hat K}
    f_k^j(u,v) \varphi_k^i(u,v) \tilde J_k(u,v) \d u \d v.
  \end{aligned}
\end{equation}


The discrete Laplace-Beltrami operator is solved for the auxiliary
vector variable $\gale$, whose finite dimensional representation is
given by $\{\gb\}$, with forcing terms given by the mean curvature
along the normal of $\tilde\Gamma$. 

In this case we write
\begin{equation*}
  [\Kb] \{\gb\} = \{\kb\},
\end{equation*}
where
\begin{equation*}
  \begin{split} 
    [\Kb] &:= 
     \begin{bmatrix}
       [K] & 0 & 0 \\
       0 & [K] & 0\\
       0 & 0 & [K]
     \end{bmatrix}\\
     \{\kb\} &:= - 2 k
     \begin{Bmatrix}
       \nb_x \\
       \nb_y \\
       \nb_z
     \end{Bmatrix}.
  \end{split}
\end{equation*}
%
and the full semi-discrete version of
Problem~(\ref{eq:continuous-problem}) reads
\begin{subequations}
  \label{eq:semi-discrete-problem}
  \begin{align}
    \label{eq:semidiscrete-bem}
    &\left[\alpha\right]\left\{\phi\right\} + \left[N\right]\left\{\phi\right\} -
    \left[D\right]\left\{\phin\right\}  &= 0 \\
    &[M][P_{\Gamma^w}]\{\phi\}' - [P_{\Gamma^w}]\{V_\phi\}& = 0 \label{eq:semidiscrete-bem-eta}\\
    &[M][P_{\Gamma^w}]\{\eta\}' - [P_{\Gamma^w}]\{V_\eta\} &= 0 \label{eq:semidiscrete-bem-phi}\\
    & [P_{\Gamma^w}]\{\phi (0)\} - [P_{\Gamma^w}]\{\phi_0\}& = 0\\ 
    &[P_{\Gamma^w}]\{\eta (0)\} - [P_{\Gamma^w}]\{\eta_0\} &= 0\\
    &[I-P_{\Gamma^w}]\{\phin \} - [I-P_{\Gamma^w}]\overline{\{\phin\}}
    &= 0\\
    &[P_{\gamma}]\{\gb\}' -[P_{\gamma}]\{\wb_g\} & =0\\
    &[\Kb]\{\gb\} - \{\kb\} &= 0 \\
    &[\mathcal P]\{\gb\} - \{\xb\} &= 0,
  \end{align}
\end{subequations}
where $\mathcal P$ is a numerical implementation of the projection
operator~(\ref{eq:projection-operator}). On the hull surface, this
operator is easily implemented analytically for simple model
hulls, such as the Wigley hull. In a more general case, it is
desirable to have an implementation of the projection operator that
works directly off the CAD files describing the surface. 

We implemented both an analytical projection (for the Wigley Hull
case) and a CAD based projection, using the OpenCASCADE
library~\cite{opencascade}, although some work is still required to
render our full discretization robust with respect to arbitrary hull
geometries.

%\subsection{The discretized system solution}

%In the framework of the Fast Multipole Algorithm application to the
%Boundary Elements Method, the fully populated matrix in the
%discretized system (\ref{eq:solvingSys}) is never assembled.

% The solving system is obtained by writing a Boundary Integral Equation on
% each node of the mesh.

% The system is solved by means of a GMRES method: starting from an
% initial guess solution, a call to the methods computing the
% matrix-vector products is performed, and the
% corresponding residual is evaluated. Such residual is employed by the GMRES
% solver in order to obtain a new estimate of the solution, which will used to
% compute the new matrix vector products, and a new residual, needed by the
% GMRES solver to update the solution. This iterative process is arrested when
% the norm of the residual is lower than a specified tolerance.    


\subsection{Time discretization}
\label{sec:time-discretization}

System~(\ref{eq:semi-discrete-problem}) can be recast in the following
form

\begin{equation}
\label{eq:dae_formulation}
  F(t, y, y') = 0,
\end{equation}
where we grouped the variables of the system in the vector $y$:
%
\begin{equation}
\label{eq:dae_unknowns}
y = \left\{\begin{array}{c}
           \left\{\xb\right\} \\
           \left\{ \phi\right\} \\
           \left\{ \phin\right\}
           \end{array}\right\}.
\end{equation}
%

Equation (\ref{eq:dae_formulation}) represents a system of nonlinear differential algebraic
equations ({DAE}), which we solve using the {IDA} package of the {SUNDIALS} OpenSource
library~\cite{sundials2005}.  As stated in the package
documentation (see p.~374 and~375 in \cite{sundials2005}):\footnote{We quoted
directly from the {SUNDIALS} documentation. However, we adjusted the notation so as to
be consistent with ours and we numbered equations according to their order in this paper.}
%
\begin{quote}
The integration method in {IDA} is variable-order,
variable-coefficient {BDF} [backward difference formula], in fixed-leading-coefficient form.
The method order ranges from 1 to 5, with the {BDF} of order $q$ given by the multistep formula
%%
  \begin{equation}
    \label{eq:bdf_of_order q}
    \sum_{i=0}^{q} \alpha_{n,i} y_{n-i} = h_n \dot{y}_n,
  \end{equation}
%%
where $y_{n}$ and $\dot{y}_{n}$ are the computed approximations to $y(t_{n})$ and $y'(t_{n})$,
respectively, and the step size is $h_{n} = t_{n} - t_{n-1}$. The coefficients $\alpha_{n,i}$ are
uniquely determined by the order $q$, and the history of the step sizes.  The application of the
{BDF} [in Eq.~\eqref{eq:bdf_of_order q}] to the {DAE} system [in Eq.~\eqref{eq:dae_formulation}]
results in a nonlinear algebraic system to be solved at each step:
%%
  \begin{equation}
    \label{eq:dae_algebraic_system}
    R(y_{n}) \equiv F\biggl(t_{n}, y_{n},  h_{n}^{-1} \sum_{i=0}^{q}
    \alpha_{n,i} y_{n-i}\biggr) = 0.
  \end{equation}
%%
Regardless of the method options, the solution of the nonlinear
system [in Eq.~\eqref{eq:dae_algebraic_system}] is accomplished with some form of Newton
iteration. This leads to a linear system for each Newton correction, of the form
%%
  \begin{equation}
    \label{eq:dae newton correction}
    J[y_{n,m+1}-y_{n,m}] = -R(y_{n,m}),
  \end{equation}
%%
where $y_{n,m}$ is the $m$th approximation to $y_{m}$. Here $J$ is  some approximation to the system Jacobian
%%
\begin{equation}
  \label{eq:dae_Jacobian}
  J = \frac{\partial R}{\partial y} = \frac{\partial F}{\partial y} +\alpha \frac{\partial F}{\partial y'},
\end{equation}
%%
where $\alpha = \alpha_{n,0}/h_{n}$. The scalar $\alpha$ changes whenever the step size or method order changes. 
\end{quote}
%
In our implementation, we assemble the residual $R(y_{n,m})$ at each
Newton correction, and let SUNDIALS compute an approximation of the Jacobian
in Eq.~(\ref{eq:dae_Jacobian}). The final system is solved using a preconditioned GMRES iterative
method (see, e.g., \cite{GolubVan-Loan-1996-a}). 

Despite the increase in computational cost due the implicit solution scheme, the DAE system
approach presents several advantages with respect to explicit resolution techniques. 
First, it is worth pointing out that among the unknowns in equation~(\ref{eq:dae_unknowns}), the
coordinates of all the grid nodes (except for the vertical coordinates of free surface nodes),
appear in the DAE system as \emph{algebraic} components, as their evolution is not described by a
differential equation, but computed through the smoothing operator. Yet, the time derivative of
such coordinates, \emph{i.e.}: the ALE velocity $\wb$ is readily available through the evaluation
of the BDF (\ref{eq:bdf_of_order q}), and can be used in the differential
Equations (\ref{eq:semidiscrete-bem-eta}) and (\ref{eq:semidiscrete-bem-phi}) which appear in the
DAE system. In particular, at each time step, the convergence of Newton
corrections (\ref{eq:dae newton correction}) ensures that the vertical velocity of the nodes is
the one corresponding to the $\wb$ velocity originated by the horizontal nodes displacement computed
by the smoothing operator. In a similar fashion, the DAE solution algorithm computes the ALE time
derivative of the velocity potential at each Newton correction. Such derivative is plugged into Bernoulli's
equation~(\ref{eq:bernoulli}) to evaluate the pressure on the whole domain boundary $\Gamma(t)$,
without requiring the solution of additional boundary value problems for $\frac{\Pa \phi}{\Pa t}$.
Finally, the resulting pressure field is integrated on the ship wet surface $\Gamma^h(t)$ to obtain the
pressure force acting on the ship. As this operation is done at the level of each Newton
correction, possible rigid motions of a hull along its six degrees of freedom can be accounted for
in a very natural way in the DAE framework, by adding the six differential equations of
motion governing the unknown rigid displacements to the DAE system. The latter ---strongly coupled---
fluid structure interaction model is currently under development and results will be presented in
future contributions.




\subsection{Adaptive mesh refinement}

The main advantages of using a Galerkin formulation for the evolution
equation of the free surface, as well as for the computation of the
full ALE deformation on the surface $\Gamma(t)$, is two-fold. On one
hand, fully unstructured meshes can be used, with an immediate
simplification in the mesh generation, and on the other hand, the a
posteriori error techniques which are rather popular in the finite
element community, can be adopted immediately in this framework,
coupled with local refinement strategies, to fully automate the mesh
generation and mesh adaptation based on the characteristic of the
solution itself, rather than on a-priori heuristic choices.

In this work, we use a modification of the gradient recovery error
estimator by Kelly, Gago, Zienkiewicz and
Babuska~\cite{kelly1983posteriori,gago1983posteriori}, a choice mostly
motivated by its simplicity (see~\cite{AinsworthOden-1997-a} for more
details on this and other error estimators).


\begin{figure}[htb!]        
\begin{tabular}{c c}
\includegraphics[width=.48\linewidth]{./figures/wigleyAdaptiveCoarse} &
\includegraphics[width=.48\linewidth]{./figures/wigleyAdaptiveRef}
\end{tabular}
\caption{A mesh refinement step. \label{fig:adaptiveMeshRef}}	
\end{figure}


At fixed intervals in time, the surface gradient of the finite element
approximation of $\phi$ is post-processed to provide a quantitative
estimate of where the approximation error may be higher. In
particular, for each cell $K$ of our triangulation we compute the
quantity
\begin{equation}
  \tau_K^2 := \frac{h}{24}\int_{\partial K} \left[ \nablab_s \phi \cdot \nb_{\partial
      K} \right ]^2 \d \gamma,
\end{equation}
where $[ \nablab_s \phi \cdot \nb_{\partial K} ]$ denotes the jump of
the surface gradient of $\phi$ across the edges of the triangulation
element $K$. The vector $\nb_{\partial K}$ is perpendicular to both
the cell normal $\nb$, and to the boundary of the element $K$, and $h$
is the diamater of the cell itself.

Roughly speaking, $\tau_K$ gives an estimate of how well the trial
space is approximating the surface gradient of $\phi$. The higher
these values, the smaller the cells should become. The estimated error
per cell $\tau_K$ is ordered, and a fixed fraction of the cells with
the highest and lowest error $\tau_K$ are flagged for refinement and
coarsening. The computational grid is then refined, ensuring that any
two neighboring cells differ for at most one refinement level. 

Standard interpolation is used to transfer all finite dimensional
solutions from one grid to another, and a geometrically consistent
mesh modification algorithm is used to collocate the new nodes
coordinates as smoothly as possible
(see~\cite{BonitoNochettoPauletti-2010-a} for a detailed explanation
of this algorithmic strategy). The resulting computational grid is
allowed to have hanging nodes, on which the finite dimensional fields
are constrained to be continuous. The degrees of freedom associated
with the hanging nodes are eliminated from the final system of
equations via a matrix condensation technique.

Most of these algorithmic strategies are based on the ones which were
already implemented in the \texttt{deal.II} finite element
library~\cite{BangerthHartmannKanschat2007} for trial spaces of finite
elements defined in two and three dimensions, and were modified to
allow their use on arbitrary surfaces embedded in three dimensions. An
example of a refinement step is presented in
Figure~\ref{fig:adaptiveMeshRef}.

After each coarsening and refinement step, the system of differential
algebraic equations is restarted with the newly interpolated solution
as initial condition. A state diagram for the entire solution process
is sketched in Figure~\ref{fig:state_diagram}.

\begin{figure}[htb!]
  \centering
  \includegraphics[width=.8\textwidth]{figures/StateDiagram}
  \caption{State Diagram}
  \label{fig:state_diagram}
\end{figure}

\section{Numerical simulations and results}

The test case presented in this work is the problem of a Wigley hull
advancing in calm water at speed $\Vb_\infty$ parallel to the
longitudinal axis, with fixed sinkage and trim. In naval engineering,
the Wigley hull is commonly used as a benchmark for the validation of
free surface flow simulations.  This is mainly due to its simple
shape, defined by the equation

\begin{equation}
y(x,z) = \frac{B}{2}\left[1- \left(\frac{2x}{L}\right)^2\right]\left[1- \left(\frac{z}{T}\right)^2\right].
\end{equation}
%
In our simulations the boat length, beam and draft values used are respectively  
$L = 2.5\ \text{m}$, $B = 0.25\ \text{m}$, and $T = 0.15625\ \text{m}$. A sketch of the
resulting hull shape is presented in Fig. \ref{fig:wigleyStrips}, which represents a
set of vertical sections of the hull. 

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.5\textwidth]{figures/wigleyStrips}
  \caption{Vertical sections of the Wigley hull used for the simulations, generated by planes
           normal to the longitudinal axis of the hull.}
  \label{fig:wigleyStrips}
\end{figure}

In the numerical simulation setup, the boat is started at rest, and
the its velocity is increased up to the desired speed $\Vb_\infty$
with a linear ramp. The simulation is then carried on until the flow
approaches a steady state solution. The presence of the ramp is not
needed for the stability and convergence of the solution, which are
also obtained imposing an impulsive start of the water past the
hull. Still, inducing slower dynamics in the first seconds of the
simulations, the linear ramp allows for higher time steps and faster
convergence.


% \begin{figure}[htb!]
%   \centering
%   \includegraphics[width=0.75\textwidth]{figures/wakeContour}
%   \includegraphics[width=0.75\textwidth]{figures/wakeMeshRef}
%   \caption{Top view of the wave elevation contour at Fr$=0.408$, and
%            corresponding mesh refinement pattern. The final mesh accounts
%            for approximately 6000 nodes.}
%   \label{fig:wakeAndMesh}
% \end{figure}


To compare the non linear free surface BEM solutions with the
experimental results presented in~\cite{mccarthy1985}, we considered
six different surge velocities $V_\infty$, corresponding to the Froude
numbers reported in Table \ref{tab:froudeNumbers}. For each of these
Froude numbers, numerical solutions were obtained using a refined and
a coarse mesh, in which the adaptive mesh refinement algorithm was
tuned in order to maintain the cell dimensions over a given minimum
value, and in order to limit the number of degrees of freedom under a
maximum value.


\begin{table}[htb]
\centering
%\small
\begin{tabular}{||c||c|c|c|c|c|c||}
\hline
\hline
$V_\infty$ &
1.2381$\ \frac{m}{s}$ & 1.3223$\ \frac{m}{s}$ & 1.4312$\ \frac{m}{s}$ &
1.5649$\ \frac{m}{s}$ & 1.7531$\ \frac{m}{s}$ & 2.0205$\ \frac{m}{s}$ \\
\hline
Fr &
0.250 & 0.267 & 0.289 & 0.316 & 0.354 & 0.408 \\
\hline
\hline
\end{tabular}
%\normalsize
\caption{Wigley hull surge velocities imposed in each numerical simulation, and the corresponding
         Froude numbers $\text{Fr} = \frac{V_\infty}{\sqrt{gL}}$.
\label{tab:froudeNumbers}}
\end{table}



\begin{figure}[htb!]
  \centering
  
  \subfigure[Fr = 0.250]{\includegraphics[width=\textwidth]{figures/Fr0250Mixed}}
  \subfigure[Fr = 0.267]{\includegraphics[width=\textwidth]{figures/Fr0267Mixed}}
  \caption{Mesh refinements and contours (I).}
  \label{fig:mesh-and-contours-1}
\end{figure}

\begin{figure}[htb!]
  \centering
  
  \subfigure[Fr = 0.289]{\includegraphics[width=\textwidth]{figures/Fr0289Mixed}}
  \subfigure[Fr = 0.316]{\includegraphics[width=\textwidth]{figures/Fr0316Mixed}}
 \caption{Mesh refinements and contours (II).}
  \label{fig:mesh-and-contours-2}
\end{figure}


\begin{figure}[htb!]
  \centering

  \subfigure[Fr = 0.354]{\includegraphics[width=\textwidth]{figures/Fr0354Mixed}}
  \subfigure[Fr = 0.408]{\includegraphics[width=\textwidth]{figures/Fr0408Mixed}}


  \caption{Mesh refinements and contours (III).}
  \label{fig:mesh-and-contours-3}
\end{figure}

A contour of the wave elevation field for the regime solution obtained
at the various Freude numbers is presented in
Figures~\ref{fig:mesh-and-contours-1}, \ref{fig:mesh-and-contours-2}
and~\ref{fig:mesh-and-contours-3}, along with the final mesh. The
pictures shows how the adaptive mesh refinement leads to an automatic
clustering of mesh cells which captures in very accurate manner the
physical characteristics of the wave patterns using a very limited
number of degrees of freedom. The final mesh is in fact only composed
by roughly 6000 nodes, but it allows for a very good reconstruction of
the Kelvin wake, which extends for several wavelengths past the
surging hull.



The simulations required 12 hrs (for the coarse meshes) to 48 hrs (for the refined meshes)
to reach the steady state solution, on single SMP nodes of the Arctur cluster of the
Italian/Slovenian interstate cooperation Exact-Lab/Arctur.

\begin{figure}[htb!]
  \centering
\begin{tabular}{c c}
  \includegraphics[width=0.48\textwidth]{figures/waterLineFr0250}&
  \includegraphics[width=0.48\textwidth]{figures/waterLineFr0267}\\
  \includegraphics[width=0.48\textwidth]{figures/waterLineFr0289}&
  \includegraphics[width=0.48\textwidth]{figures/waterLineFr0316}\\
  \includegraphics[width=0.48\textwidth]{figures/waterLineFr0354}&
  \includegraphics[width=0.48\textwidth]{figures/waterLineFr0408}
\end{tabular}

  \caption{Comparison of predicted water profiles with the University of Tokyo
           experimental results ({\color{black}- -$\ast$- -}). Both coarse
           mesh ({\color{red}-- --}) and refined mesh results ({\color{blue}---})
           are shown in the plots.}
  \label{fig:waterLine}
\end{figure}


The wave profiles on the surface of the Wigley hull obtained with the
present method, are compared with the corresponding experimental
results in Fig. \ref{fig:waterLine}. In each plot, the abscissae
represent the dimensionless coordinate $x/L$ along the boat, while the
ordinates are the dimensionless wave elevations $\eta ' =
\frac{2g\eta}{{V_\infty}^2}$. For all the Froude numbers considered,
the method presented seems able to predict qualitatively correct wave
profiles. Moreover, the wave elevation in proximity of the bow of the
boat is reproduced with very good accuracy in all the test cases
considered. On the other hand, in all the numerical curves, we can
observe a small spatial oscillation superimposed to the main wave
profile. The wave length of such oscillation seems proportional to the
local mesh cells size, while the amplitude is slightly higher for
finer meshes, suggesting that better tuning of the SUPG stabilization
parameter may be needed for this kind of boundary value
problems. % This might
% suggest that the SUPG stabilization is not completely removing the numerical instability
% due to the dominant transport term in the free surface equations. For this reason,
% investigations on a more suitable tuning of the characteristic lenght appearing in the
% SUPG shape function formulation is underway.   

\section{Conclusions}
\label{sec:conclusions}

An accurate and efficient boundary element method for the simulation
of unsteady and fully nonlinear potential waves past surging ships was
developed, implemented and tested. Compared to existing algorithms,
the method presents several innovative aspects which try to address
some of the most CPU intensive aspects of this kind of computations.

The most innovative idea behind the proposed method is the fact that
the equations are studied on a fixed reference domain, which is
deformed through an arbitrary Lagrangian Eulerian map that keeps track
of the physical shape of the water domain around the ship. Some
aspects of this approach resemble the semi-Lagrangian formulation of
the potential wave equations, but here they are takled using powerful
differential geometry tools, combined with finite element techniques
for arbitrary surfaces.

This reformulation in terms of a fixed reference domain presents
severe stability issues in presence of a forward ship motion, or in
presence of an incident stream velocity. Stabilization is achieved via
a weighted SUPG projection, which allows the use of fully unstructured
meshes, and guarantees an accurate reconstruction of the velocity
fields on the mesh nodes, also when low order finite dimensional
spaces are used for the numerical discretization.

To the best of the authors' knowledge, such formulation has never been
successfully used in ship hydrodynamic problems in presence of a non
zero stream velocity, due to the free surface instabilities.
 
With respect to existing methods, the combination of the
semi-Lagrangian approach with the SUPG stabilization eliminates the
need for periodic remeshing of the computational domain, and opens up
the possibility to exploit local adaptivity tools, typical of finite
element discretizations.

We exploit these ideas by employing simple a posteriori error
estimates to adaptively refine the computational mesh, in order to
automatically follow the characteristics of the computed
solution. Accurate results are obtained even when using a very limited
number of degrees of freedom.

Implicit BDF methods with variable order and variable step size are
also employed, which render the final computational tool very
attractive in terms of robustness. 

A direct interface with standard CAD file formats is currently under
development, and our preliminary results indicate that the final tool
could be used to efficiently study the unsteady interaction between
arbitrary hull shapes and nonlinear water waves in a robust and
automated way.

\section*{Acknowledgments}
\label{sec:aknowledgments}

The research leading to these results has received specific funding
under the ``Young SISSA Scientists' Research Projects'' scheme
2011-2012, promoted by the International School for Advanced Studies
(SISSA), Trieste, Italy.

This work was performed in the context of the project OpenSHIP,
``Simulazioni di fluidodinamica computazionale (CFD) di alta qualita per
le previsioni di prestazioni idrodinamiche del sistema carena-elica in
ambiente OpenSOURCE'', supported by Regione FVG - POR FESR 2007-2013
Obiettivo competitivita regionale e occupazione.

The authors gratefully acknowledge the Italian/Slovenian cross-border
cooperation eXact-Lab/Arctur for the processing power that was made
available on the Arctur cluster.

\bibliographystyle{plain}
\bibliography{References}


\end{document}

